Explainability of deep vision-based autonomous driving systems: Review and challenges

This survey reviews explainability methods for vision-based self-driving systems trained with behavior cloning. The concept of explainability has several facets and the need for explainability is strong in driving, a safety-critical application. Gathering contributions from several research fields, namely computer vision, deep learning, autonomous driving, explainable AI (X-AI), this survey tackles several points. First, it discusses definitions, context, and motivation for gaining more interpretability and explainability from self-driving systems, as well as the challenges that are specific to this application. Second, methods providing explanations to a black-box self-driving system in a post-hoc fashion are comprehensively organized and detailed. Third, approaches from the literature that aim at building more interpretable self-driving systems by design are presented and discussed in detail. Finally, remaining open-challenges and potential future research directions are identified and examined.

==> biblio_copy.tex <==
@string{bmvc={Proceedings of the British Machine Vision Conference (BMVC)}}
@string{cviu={Computer Vision and Image Understanding (CVIU)}}
@string{cvpr={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}}
@string{eccv={Proceedings of the IEEE European Conference on Computer Vision (ECCV)}}
@string{iccv={Proceedings of the IEEE International Conference on Computer Vision (ICCV)}}
@string{iclr={Proceedings of the International Conference on Learning Representations (ICLR)}}
@string{ijcv={International Journal of Computer Vision (IJCV)}}
@string{nips={Advances in Neural Information Processing Systems (NIPS)}}
@string{tpami={IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)}}
@string{aaai={Proceedings of the AAAI Conference on Artificial Intelligence (AAAI)}}
@string{emnlp={Proceedings of the Conference on Empirical Methods in Natural Language Processing (EMNLP)}}

@article{RosenfeldR19,
  author    = {Avi Rosenfeld and
               Ariella Richardson},
  title     = {Explainability in human-agent systems},
  journal   = {Auton. Agents Multi Agent Syst.},
  volume    = {33},
  number    = {6},
  pages     = {673--705},
  year      = {2019},
  url       = {https://doi.org/10.1007/s10458-019-09408-y},
  doi       = {10.1007/s10458-019-09408-y},
  timestamp = {Fri, 13 Mar 2020 10:55:56 +0100},
  biburl    = {https://dblp.org/rec/journals/aamas/RosenfeldR19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{GilpinBYBSK18,
  author    = {Leilani H. Gilpin and
               David Bau and
               Ben Z. Yuan and
               Ayesha Bajwa and
               Michael Specter and
               Lalana Kagal},
  editor    = {Francesco Bonchi and
               Foster J. Provost and
               Tina Eliassi{-}Rad and
               Wei Wang and
               Ciro Cattuto and
               Rayid Ghani},
  title     = {Explaining Explanations: An Overview of Interpretability of Machine
               Learning},
  booktitle = {5th {IEEE} International Conference on Data Science and Advanced Analytics,
               {DSAA} 2018, Turin, Italy, October 1-3, 2018},
  pages     = {80--89},
  publisher = {{IEEE}},
  year      = {2018},
  url       = {https://doi.org/10.1109/DSAA.2018.00018},
  doi       = {10.1109/DSAA.2018.00018},
  timestamp = {Wed, 16 Oct 2019 14:14:55 +0200},
  biburl    = {https://dblp.org/rec/conf/dsaa/GilpinBYBSK18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{10.1145/3236009,
author = {Guidotti, Riccardo and Monreale, Anna and Ruggieri, Salvatore and Turini, Franco and Giannotti, Fosca and Pedreschi, Dino},
title = {A Survey of Methods for Explaining Black Box Models},
year = {2018},
issue_date = {January 2019},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {51},
number = {5},
issn = {0360-0300},
url = {https://doi.org/10.1145/3236009},
doi = {10.1145/3236009},
journal = {ACM Comput. Surv.},
month = aug,
articleno = {93},
numpages = {42},
keywords = {explanations, Open the black box, transparent models, interpretability}
}
  
@article{doshi2017accountability,
  title={Accountability of AI Under the Law: The Role of Explanation},
  author={Doshi-Velez, Finale and Kortz, Mason A},
  year={2017},
  publisher={Berkman Klein Center for Internet \& Society}
}

@inproceedings{desire,
  author    = {Namhoon Lee and
               Wongun Choi and
               Paul Vernaza and
               Christopher B. Choy and
               Philip H. S. Torr and
               Manmohan Chandraker},
  title     = {{DESIRE:} Distant Future Prediction in Dynamic Scenes with Interacting
               Agents},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {2165--2174},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.233},
  doi       = {10.1109/CVPR.2017.233},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/LeeCVCTC17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
a service of Schloss Dagstuhl - Leibniz Center for Informatics	homebrowsesearchabout
w3c valid html last updat

@inproceedings{textual_explanations,
  author    = {Jinkyu Kim and
               Anna Rohrbach and
               Trevor Darrell and
               John F. Canny and
               Zeynep Akata},
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {Textual Explanations for Self-Driving Vehicles},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {II}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11206},
  pages     = {577--593},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-01216-8\_35},
  doi       = {10.1007/978-3-030-01216-8\_35},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/KimRDCA18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{pilotnet,
  author    = {Mariusz Bojarski and
               Davide Del Testa and
               Daniel Dworakowski and
               Bernhard Firner and
               Beat Flepp and
               Prasoon Goyal and
               Lawrence D. Jackel and
               Mathew Monfort and
               Urs Muller and
               Jiakai Zhang and
               Xin Zhang and
               Jake Zhao and
               Karol Zieba},
  title     = {End to End Learning for Self-Driving Cars},
  journal   = {CoRR},
  volume    = {abs/1604.07316},
  year      = {2016},
  url       = {http://arxiv.org/abs/1604.07316},
  archivePrefix = {arXiv},
  eprint    = {1604.07316},
  timestamp = {Mon, 13 Aug 2018 16:47:06 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/BojarskiTDFFGJM16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{du2019look,
  title={Look who’s talking now: Implications of AV’s explanations on driver’s trust, AV preference, anxiety and mental workload},
  author={Du, Na and Haspiel, Jacob and Zhang, Qiaoning and Tilbury, Dawn and Pradhan, Anuj K and Yang, X Jessie and Robert Jr, Lionel P},
  journal={Transportation research part C: emerging technologies},
  volume={104},
  pages={428--442},
  year={2019},
  publisher={Elsevier}
}

@article{shen2020explain,
  author    = {Yuan Shen and
               Shanduojiao Jiang and
               Yanlin Chen and
               Eileen Yang and
               Xilun Jin and
               Yuliang Fan and
               Katie Driggs Campbell},
  title     = {To Explain or Not to Explain: {A} Study on the Necessity of Explanations
               for Autonomous Vehicles},
  journal   = {CoRR},
  volume    = {abs/2006.11684},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.11684},
  archivePrefix = {arXiv},
  eprint    = {2006.11684},
  timestamp = {Tue, 23 Jun 2020 17:57:22 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-11684.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{trusthci20,
  author    = {Qiaoning Zhang and
               X. Jessie Yang and
               Lionel Peter Robert},
  editor    = {Regina Bernhaupt and
               Florian 'Floyd' Mueller and
               David Verweij and
               Josh Andres and
               Joanna McGrenere and
               Andy Cockburn and
               Ignacio Avellino and
               Alix Goguey and
               Pernille Bj{\o}n and
               Shengdong Zhao and
               Briane Paul Samson and
               Rafal Kocielnik},
  title     = {Expectations and Trust in Automated Vehicles},
  booktitle = {Extended Abstracts of the 2020 {CHI} Conference on Human Factors in
               Computing Systems, {CHI} 2020, Honolulu, HI, USA, April 25-30, 2020},
  pages     = {1--9},
  publisher = {{ACM}},
  year      = {2020},
  url       = {https://doi.org/10.1145/3334480.3382986},
  doi       = {10.1145/3334480.3382986},
  timestamp = {Tue, 12 May 2020 15:39:28 +0200},
  biburl    = {https://dblp.org/rec/conf/chi/ZhangYR20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{trusthci15,
  author    = {Jong Kyu Choi and
               Yong Gu Ji},
  title     = {Investigating the Importance of Trust on Adopting an Autonomous Vehicle},
  journal   = {Int. J. Hum. Comput. Interact.},
  volume    = {31},
  number    = {10},
  pages     = {692--702},
  year      = {2015},
  url       = {https://doi.org/10.1080/10447318.2015.1070549},
  doi       = {10.1080/10447318.2015.1070549},
  timestamp = {Thu, 18 Jun 2020 22:01:59 +0200},
  biburl    = {https://dblp.org/rec/journals/ijhci/ChoiJ15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{shapgdpr,
  author    = {Shubham Rathi},
  title     = {Generating Counterfactual and Contrastive Explanations using {SHAP}},
  journal   = {CoRR},
  volume    = {abs/1906.09293},
  year      = {2019},
  url       = {http://arxiv.org/abs/1906.09293},
  archivePrefix = {arXiv},
  eprint    = {1906.09293},
  timestamp = {Thu, 27 Jun 2019 18:54:51 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1906-09293.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{thrun2006stanley,
  title={Stanley: The robot that won the DARPA Grand Challenge},
  author={Thrun, Sebastian and Montemerlo, Mike and Dahlkamp, Hendrik and Stavens, David and Aron, Andrei and Diebel, James and Fong, Philip and Gale, John and Halpenny, Morgan and Hoffmann, Gabriel and others},
  journal={Journal of field Robotics},
  volume={23},
  number={9},
  pages={661--692},
  year={2006},
  publisher={Wiley Online Library}
}
@article{urmson2008autonomous,
  title={Autonomous driving in urban environments: Boss and the urban challenge},
  author={Urmson, Chris and Anhalt, Joshua and Bagnell, Drew and Baker, Christopher and Bittner, Robert and Clark, MN and Dolan, John and Duggins, Dave and Galatali, Tugrul and Geyer, Chris and others},
  journal={Journal of Field Robotics},
  volume={25},
  number={8},
  pages={425--466},
  year={2008},
  publisher={Wiley Online Library}
}

@inproceedings{DBLP:conf/itsc/AkaiSYTYOSN17,
  author    = {Naoki Akai and
               Luis Yoichi Morales Saiki and
               Takuma Yamaguchi and
               Eijiro Takeuchi and
               Yuki Yoshihara and
               Hiroyuki Okuda and
               Tatsuya Suzuki and
               Yoshiki Ninomiya},
  title     = {Autonomous driving based on accurate localization using multilayer
               LiDAR and dead reckoning},
  booktitle = {20th {IEEE} International Conference on Intelligent Transportation
               Systems, {ITSC} 2017, Yokohama, Japan, October 16-19, 2017},
  pages     = {1--6},
  year      = {2017},
  crossref  = {DBLP:conf/itsc/2017},
  url       = {https://doi.org/10.1109/ITSC.2017.8317797},
  doi       = {10.1109/ITSC.2017.8317797},
  timestamp = {Wed, 16 Oct 2019 14:14:57 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/itsc/AkaiSYTYOSN17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/ijcai/McAllisterGKWSC17,
  author    = {Rowan McAllister and
               Yarin Gal and
               Alex Kendall and
               Mark van der Wilk and
               Amar Shah and
               Roberto Cipolla and
               Adrian Weller},
  title     = {Concrete Problems for Autonomous Vehicle Safety: Advantages of Bayesian
               Deep Learning},
  booktitle = {Proceedings of the Twenty-Sixth International Joint Conference on
               Artificial Intelligence, {IJCAI} 2017, Melbourne, Australia, August
               19-25, 2017},
  pages     = {4745--4753},
  year      = {2017},
  crossref  = {DBLP:conf/ijcai/2017},
  url       = {https://doi.org/10.24963/ijcai.2017/661},
  doi       = {10.24963/ijcai.2017/661},
  timestamp = {Tue, 20 Aug 2019 16:19:23 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/ijcai/McAllisterGKWSC17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/nips/Pomerleau88,
  author    = {Dean Pomerleau},
  title     = {{ALVINN:} An Autonomous Land Vehicle in a Neural Network},
  booktitle = {Advances in Neural Information Processing Systems 1, {[NIPS} Conference,
               Denver, Colorado, USA, 1988]},
  pages     = {305--313},
  year      = {1988},
  crossref  = {DBLP:conf/nips/1988},
  url       = {http://papers.nips.cc/paper/95-alvinn-an-autonomous-land-vehicle-in-a-neural-network},
  timestamp = {Thu, 11 Dec 2014 17:34:07 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/nips/Pomerleau88},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1906-05113,
  author    = {Ekim Yurtsever and
               Jacob Lambert and
               Alexander Carballo and
               Kazuya Takeda},
  title     = {A Survey of Autonomous Driving: Common Practices and Emerging Technologies},
  journal   = {CoRR},
  volume    = {abs/1906.05113},
  year      = {2019},
  url       = {http://arxiv.org/abs/1906.05113},
  archivePrefix = {arXiv},
  eprint    = {1906.05113},
  timestamp = {Fri, 14 Jun 2019 09:38:24 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1906-05113},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{bddv,
  author    = {Huazhe Xu and
               Yang Gao and
               Fisher Yu and
               Trevor Darrell},
  title     = {End-to-End Learning of Driving Models from Large-Scale Video Datasets},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {3530--3538},
  year      = {2017},
  crossref  = {DBLP:conf/cvpr/2017},
  url       = {https://doi.org/10.1109/CVPR.2017.376},
  doi       = {10.1109/CVPR.2017.376},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/XuGYD17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{codevilla2018end,
  title={End-to-end driving via conditional imitation learning},
  author={Codevilla, Felipe and Miiller, Matthias and L{\'o}pez, Antonio and Koltun, Vladlen and Dosovitskiy, Alexey},
  booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={1--9},
  year={2018},
  organization={IEEE}
}

@inproceedings{codevilla2019exploring,
  title={Exploring the limitations of behavior cloning for autonomous driving},
  author={Codevilla, Felipe and Santana, Eder and L{\'o}pez, Antonio M and Gaidon, Adrien},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={9329--9338},
  year={2019}
}

@InProceedings{Buhet_2019_ICCV,
author = {Buhet, Thibault and Wirbel, Emilie and Perrotton, Xavier},
title = {Conditional Vehicle Trajectories Prediction in CARLA Urban Environment},
booktitle = {The IEEE International Conference on Computer Vision (ICCV) Workshops},
month = {Oct},
year = {2019}
}

@inproceedings{deepdrivingaffordance,
  author    = {Chenyi Chen and
               Ari Seff and
               Alain L. Kornhauser and
               Jianxiong Xiao},
  title     = {DeepDriving: Learning Affordance for Direct Perception in Autonomous
               Driving},
  booktitle = {2015 {IEEE} International Conference on Computer Vision, {ICCV} 2015,
               Santiago, Chile, December 7-13, 2015},
  pages     = {2722--2730},
  publisher = {{IEEE} Computer Society},
  year      = {2015},
  url       = {https://doi.org/10.1109/ICCV.2015.312},
  doi       = {10.1109/ICCV.2015.312},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iccv/ChenSKX15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{conditionalaffordance,
  author    = {Axel Sauer and
               Nikolay Savinov and
               Andreas Geiger},
  title     = {Conditional Affordance Learning for Driving in Urban Environments},
  booktitle = {2nd Annual Conference on Robot Learning, CoRL 2018, Z{\"{u}}rich,
               Switzerland, 29-31 October 2018, Proceedings},
  series    = {Proceedings of Machine Learning Research},
  volume    = {87},
  pages     = {237--252},
  publisher = {{PMLR}},
  year      = {2018},
  url       = {http://proceedings.mlr.press/v87/sauer18a.html},
  timestamp = {Wed, 03 Apr 2019 18:17:24 +0200},
  biburl    = {https://dblp.org/rec/conf/corl/SauerSG18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{guidedsupervision,
  author    = {Ashish Mehta and
               Adithya Subramanian and
               Anbumani Subramanian},
  title     = {Learning End-to-end Autonomous Driving using Guided Auxiliary Supervision},
  booktitle = {{ICVGIP} 2018: 11th Indian Conference on Computer Vision, Graphics
               and Image Processing, Hyderabad, India, 18-22 December, 2018},
  pages     = {11:1--11:8},
  publisher = {{ACM}},
  year      = {2018},
  url       = {https://doi.org/10.1145/3293353.3293364},
  doi       = {10.1145/3293353.3293364},
  timestamp = {Thu, 07 May 2020 12:10:48 +0200},
  biburl    = {https://dblp.org/rec/conf/icvgip/MehtaSS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{marinaffordance,
  author    = {Marin Toromanoff and
               {\'{E}}milie Wirbel and
               Fabien Moutarde},
  title     = {End-to-End Model-Free Reinforcement Learning for Urban Driving using
               Implicit Affordances},
  journal   = {CoRR},
  volume    = {abs/1911.10868},
  year      = {2019},
  url       = {http://arxiv.org/abs/1911.10868},
  archivePrefix = {arXiv},
  eprint    = {1911.10868},
  timestamp = {Tue, 03 Dec 2019 14:15:54 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1911-10868.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{lee1992trust,
  title={Trust, control strategies and allocation of function in human-machine systems},
  author={Lee, John and Moray, Neville},
  journal={Ergonomics},
  volume={35},
  number={10},
  pages={1243--1270},
  year={1992},
  publisher={Taylor \& Francis}
}

@article{lee1994trust,
  title={Trust, self-confidence, and operators' adaptation to automation},
  author={Lee, John D and Moray, Neville},
  journal={International journal of human-computer studies},
  volume={40},
  number={1},
  pages={153--184},
  year={1994},
  publisher={Elsevier}
}

@article{sheridan1975considerations,
  title={Considerations in modeling the human supervisory controller},
  author={Sheridan, Thomas B},
  journal={IFAC Proceedings Volumes},
  volume={8},
  number={1},
  pages={223--228},
  year={1975},
  publisher={Elsevier}
}

@techreport{sheridan1984research,
  title={Research and modeling of supervisory control behavior. Report of a workshop},
  author={Sheridan, Thomas B and Hennessy, Robert T},
  year={1984},
  institution={National research council Washington DC committee on human factors}
}

download as .bib file

@inproceedings{hasan2012trust,
  author    = {Zahid Hasan and
               Alina Krischkowsky and
               Manfred Tscheligi},
  editor    = {Stefan Katzenbeisser and
               Edgar R. Weippl and
               L. Jean Camp and
               Melanie Volkamer and
               Mike K. Reiter and
               Xinwen Zhang},
  title     = {Modelling User-Centered-Trust {(UCT)} in Software Systems: Interplay
               of Trust, Affect and Acceptance Model},
  booktitle = {Trust and Trustworthy Computing - 5th International Conference, {TRUST}
               2012, Vienna, Austria, June 13-15, 2012. Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {7344},
  pages     = {92--109},
  publisher = {Springer},
  year      = {2012},
  url       = {https://doi.org/10.1007/978-3-642-30921-2\_6},
  doi       = {10.1007/978-3-642-30921-2\_6},
  timestamp = {Tue, 14 May 2019 10:00:51 +0200},
  biburl    = {https://dblp.org/rec/conf/trust/HasanKT12.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@book{anderson2014autonomous,
  title={Autonomous vehicle technology: A guide for policymakers},
  author={Anderson, James M and Nidhi, Kalra and Stanley, Karlyn D and Sorensen, Paul and Samaras, Constantine and Oluwatola, Oluwatobi A},
  year={2014},
  publisher={Rand Corporation}
}

@article{bansal2016assessing,
  title={Assessing public opinions of and interest in new vehicle technologies: An Austin perspective},
  author={Bansal, Prateek and Kockelman, Kara M and Singh, Amit},
  journal={Transportation Research Part C: Emerging Technologies},
  volume={67},
  pages={1--14},
  year={2016},
  publisher={Elsevier}
}

@inproceedings{haspiel2018explanations,
  author    = {Jacob Haspiel and
               Na Du and
               Jill Meyerson and
               Lionel P. Robert Jr. and
               Dawn M. Tilbury and
               X. Jessie Yang and
               Anuj K. Pradhan},
  editor    = {Takayuki Kanda and
               Selma Sabanovic and
               Guy Hoffman and
               Adriana Tapus},
  title     = {Explanations and Expectations: Trust Building in Automated Vehicles},
  booktitle = {Companion of the 2018 {ACM/IEEE} International Conference on Human-Robot
               Interaction, {HRI} 2018, Chicago, IL, USA, March 05-08, 2018},
  pages     = {119--120},
  publisher = {{ACM}},
  year      = {2018},
  url       = {https://doi.org/10.1145/3173386.3177057},
  doi       = {10.1145/3173386.3177057},
  timestamp = {Wed, 25 Sep 2019 18:09:14 +0200},
  biburl    = {https://dblp.org/rec/conf/hri/HaspielDMRTYP18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/hri/JayaramanCRTYPT18,
  author    = {Suresh Kumaar Jayaraman and
               Chandler Creech and
               Lionel P. Robert Jr. and
               Dawn M. Tilbury and
               X. Jessie Yang and
               Anuj K. Pradhan and
               Katherine M. Tsui},
  editor    = {Takayuki Kanda and
               Selma Sabanovic and
               Guy Hoffman and
               Adriana Tapus},
  title     = {Trust in {AV:} An Uncertainty Reduction Model of AV-Pedestrian Interactions},
  booktitle = {Companion of the 2018 {ACM/IEEE} International Conference on Human-Robot
               Interaction, {HRI} 2018, Chicago, IL, USA, March 05-08, 2018},
  pages     = {133--134},
  publisher = {{ACM}},
  year      = {2018},
  url       = {https://doi.org/10.1145/3173386.3177073},
  doi       = {10.1145/3173386.3177073},
  timestamp = {Sat, 19 Oct 2019 20:11:32 +0200},
  biburl    = {https://dblp.org/rec/conf/hri/JayaramanCRTYPT18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{kyriakidis2015public,
  title={Public opinion on automated driving: Results of an international questionnaire among 5000 respondents},
  author={Kyriakidis, Miltos and Happee, Riender and de Winter, Joost CF},
  journal={Transportation research part F: traffic psychology and behaviour},
  volume={32},
  pages={127--140},
  year={2015},
  publisher={Elsevier}
}

@article{ruijten2018enhancing,
  title={Enhancing trust in autonomous vehicles through intelligent user interfaces that mimic human behavior},
  author={Ruijten, Peter AM and Terken, Jacques and Chandramouli, Sanjeev N},
  journal={Multimodal Technologies and Interaction},
  volume={2},
  number={4},
  pages={62},
  year={2018},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{DBLP:journals/hf/HoffB15,
  author    = {Kevin Anthony Hoff and
               Masooda Bashir},
  title     = {Trust in Automation: Integrating Empirical Evidence on Factors That
               Influence Trust},
  journal   = {Hum. Factors},
  volume    = {57},
  number    = {3},
  pages     = {407--434},
  year      = {2015},
  url       = {https://doi.org/10.1177/0018720814547570},
  doi       = {10.1177/0018720814547570},
  timestamp = {Thu, 04 Jun 2020 19:43:47 +0200},
  biburl    = {https://dblp.org/rec/journals/hf/HoffB15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iui/PuC06,
  author    = {Pearl Pu and
               Li Chen},
  editor    = {C{\'{e}}cile Paris and
               Candace L. Sidner},
  title     = {Trust building with explanation interfaces},
  booktitle = {Proceedings of the 11th International Conference on Intelligent User
               Interfaces, {IUI} 2006, Sydney, Australia, January 29 - February 1,
               2006},
  pages     = {93--100},
  publisher = {{ACM}},
  year      = {2006},
  url       = {https://doi.org/10.1145/1111449.1111475},
  doi       = {10.1145/1111449.1111475},
  timestamp = {Tue, 06 Nov 2018 11:07:41 +0100},
  biburl    = {https://dblp.org/rec/conf/iui/PuC06.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{waytz2014mind,
  title={The mind in the machine: Anthropomorphism increases trust in an autonomous vehicle},
  author={Waytz, Adam and Heafner, Joy and Epley, Nicholas},
  journal={Journal of Experimental Social Psychology},
  volume={52},
  pages={113--117},
  year={2014},
  publisher={Elsevier}
}

@incollection{khastgir2017calibrating,
  title={Calibrating trust to increase the use of automated systems in a vehicle},
  author={Khastgir, Siddartha and Birrell, Stewart and Dhadyalla, Gunwant and Jennings, Paul},
  booktitle={Advances in human aspects of transportation},
  pages={535--546},
  year={2017},
  publisher={Springer}
}

@inproceedings{DBLP:conf/chi/WiegandSWLH19,
  author    = {Gesa Wiegand and
               Matthias Schmidmaier and
               Thomas Weber and
               Yuanting Liu and
               Heinrich Hussmann},
  editor    = {Regan L. Mandryk and
               Stephen A. Brewster and
               Mark Hancock and
               Geraldine Fitzpatrick and
               Anna L. Cox and
               Vassilis Kostakos and
               Mark Perry},
  title     = {I Drive - You Trust: Explaining Driving Behavior Of Autonomous Cars},
  booktitle = {Extended Abstracts of the 2019 {CHI} Conference on Human Factors in
               Computing Systems, {CHI} 2019, Glasgow, Scotland, UK, May 04-09, 2019},
  publisher = {{ACM}},
  year      = {2019},
  url       = {https://doi.org/10.1145/3290607.3312817},
  doi       = {10.1145/3290607.3312817},
  timestamp = {Fri, 03 May 2019 10:46:38 +0200},
  biburl    = {https://dblp.org/rec/conf/chi/WiegandSWLH19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{beaudouin2020identifying,
  author    = {Val{\'{e}}rie Beaudouin and
               Isabelle Bloch and
               David Bounie and
               St{\'{e}}phan Cl{\'{e}}men{\c{c}}on and
               Florence d'Alch{\'{e}}{-}Buc and
               James Eagan and
               Winston Maxwell and
               Pavlo Mozharovskyi and
               Jayneel Parekh},
  title     = {Flexible and Context-Specific {AI} Explainability: {A} Multidisciplinary
               Approach},
  journal   = {CoRR},
  volume    = {abs/2003.07703},
  year      = {2020},
  url       = {https://arxiv.org/abs/2003.07703},
  archivePrefix = {arXiv},
  eprint    = {2003.07703},
  timestamp = {Tue, 24 Mar 2020 16:42:29 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2003-07703.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{camburu2019,
  author    = {Oana{-}Maria Camburu and
               Eleonora Giunchiglia and
               Jakob Foerster and
               Thomas Lukasiewicz and
               Phil Blunsom},
  title     = {Can {I} Trust the Explainer? Verifying Post-hoc Explanatory Methods},
  journal   = {CoRR},
  volume    = {abs/1910.02065},
  year      = {2019},
  url       = {http://arxiv.org/abs/1910.02065},
  archivePrefix = {arXiv},
  eprint    = {1910.02065},
  timestamp = {Wed, 09 Oct 2019 14:07:58 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1910-02065.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{whomakedriversstop,
  author    = {Chengxi Li and
               Stanley H. Chan and
               Yi{-}Ting Chen},
  title     = {Who Make Drivers Stop? Towards Driver-centric Risk Assessment: Risk
               Object Identification via Causal Inference},
  journal   = {CoRR},
  volume    = {abs/2003.02425},
  year      = {2020},
  url       = {https://arxiv.org/abs/2003.02425},
  archivePrefix = {arXiv},
  eprint    = {2003.02425},
  timestamp = {Tue, 10 Mar 2020 13:33:48 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2003-02425.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{cultrera2020,
  author    = {Luca Cultrera and
               Lorenzo Seidenari and
               Federico Becattini and
               Pietro Pala and
               Alberto Del Bimbo},
  title     = {Explaining Autonomous Driving by Learning End-to-End Visual Attention},
  journal   = {CoRR},
  volume    = {abs/2006.03347},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.03347},
  archivePrefix = {arXiv},
  eprint    = {2006.03347},
  timestamp = {Mon, 08 Jun 2020 15:48:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-03347.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{attention_branch_network,
  author    = {Keisuke Mori and
               Hiroshi Fukui and
               Takuya Murase and
               Tsubasa Hirakawa and
               Takayoshi Yamashita and
               Hironobu Fujiyoshi},
  title     = {Visual Explanation by Attention Branch Network for End-to-end Learning-based
               Self-driving},
  booktitle = {2019 {IEEE} Intelligent Vehicles Symposium, {IV} 2019, Paris, France,
               June 9-12, 2019},
  pages     = {1577--1582},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/IVS.2019.8813900},
  doi       = {10.1109/IVS.2019.8813900},
  timestamp = {Wed, 16 Oct 2019 14:14:57 +0200},
  biburl    = {https://dblp.org/rec/conf/ivs/MoriFMHYF19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{model_failure_saliency_maps,
  author    = {Sina Mohseni and
               Akshay Jagadeesh and
               Zhangyang Wang},
  title     = {Predicting Model Failure using Saliency Maps in Autonomous Driving
               Systems},
  journal   = {CoRR},
  volume    = {abs/1905.07679},
  year      = {2019},
  url       = {http://arxiv.org/abs/1905.07679},
  archivePrefix = {arXiv},
  eprint    = {1905.07679},
  timestamp = {Tue, 28 May 2019 12:48:08 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1905-07679.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{chen2019brain,
  author    = {Shi{-}tao Chen and
               Songyi Zhang and
               Jinghao Shang and
               Badong Chen and
               Nanning Zheng},
  title     = {Brain-Inspired Cognitive Model With Attention for Self-Driving Cars},
  journal   = {{IEEE} Trans. Cogn. Dev. Syst.},
  volume    = {11},
  number    = {1},
  pages     = {13--25},
  year      = {2019},
  url       = {https://doi.org/10.1109/TCDS.2017.2717451},
  doi       = {10.1109/TCDS.2017.2717451},
  timestamp = {Fri, 06 Mar 2020 21:55:38 +0100},
  biburl    = {https://dblp.org/rec/journals/tamd/ChenZSCZ19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{causal_attention,
  author    = {Jinkyu Kim and
               John F. Canny},
  title     = {Interpretable Learning for Self-Driving Cars by Visualizing Causal
               Attention},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2017, Venice,
               Italy, October 22-29, 2017},
  pages     = {2961--2969},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/ICCV.2017.320},
  doi       = {10.1109/ICCV.2017.320},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iccv/KimC17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{l2x,
  author    = {Jianbo Chen and
               Le Song and
               Martin J. Wainwright and
               Michael I. Jordan},
  editor    = {Jennifer G. Dy and
               Andreas Krause},
  title     = {Learning to Explain: An Information-Theoretic Perspective on Model
               Interpretation},
  booktitle = {Proceedings of the 35th International Conference on Machine Learning,
               {ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July
               10-15, 2018},
  series    = {Proceedings of Machine Learning Research},
  volume    = {80},
  pages     = {882--891},
  publisher = {{PMLR}},
  year      = {2018},
  url       = {http://proceedings.mlr.press/v80/chen18j.html},
  timestamp = {Wed, 03 Apr 2019 18:17:30 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/ChenSWJ18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{shap,
  author    = {Scott M. Lundberg and
               Su{-}In Lee},
  editor    = {Isabelle Guyon and
               Ulrike von Luxburg and
               Samy Bengio and
               Hanna M. Wallach and
               Rob Fergus and
               S. V. N. Vishwanathan and
               Roman Garnett},
  title     = {A Unified Approach to Interpreting Model Predictions},
  booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
               on Neural Information Processing Systems 2017, 4-9 December 2017,
               Long Beach, CA, {USA}},
  pages     = {4765--4774},
  year      = {2017},
  url       = {http://papers.nips.cc/paper/7062-a-unified-approach-to-interpreting-model-predictions},
  timestamp = {Fri, 06 Mar 2020 16:56:21 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/LundbergL17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{lime,
  author    = {Marco T{\'{u}}lio Ribeiro and
               Sameer Singh and
               Carlos Guestrin},
  editor    = {Balaji Krishnapuram and
               Mohak Shah and
               Alexander J. Smola and
               Charu C. Aggarwal and
               Dou Shen and
               Rajeev Rastogi},
  title     = {"Why Should {I} Trust You?": Explaining the Predictions of Any Classifier},
  booktitle = {Proceedings of the 22nd {ACM} {SIGKDD} International Conference on
               Knowledge Discovery and Data Mining, San Francisco, CA, USA, August
               13-17, 2016},
  pages     = {1135--1144},
  publisher = {{ACM}},
  year      = {2016},
  url       = {https://doi.org/10.1145/2939672.2939778},
  doi       = {10.1145/2939672.2939778},
  timestamp = {Tue, 06 Nov 2018 16:59:37 +0100},
  biburl    = {https://dblp.org/rec/conf/kdd/Ribeiro0G16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{xaimedical,
  author    = {Erico Tjoa and
               Cuntai Guan},
  title     = {A Survey on Explainable Artificial Intelligence {(XAI):} Towards Medical
               {XAI}},
  journal   = {CoRR},
  volume    = {abs/1907.07374},
  year      = {2019},
  url       = {http://arxiv.org/abs/1907.07374},
  archivePrefix = {arXiv},
  eprint    = {1907.07374},
  timestamp = {Tue, 23 Jul 2019 10:54:22 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1907-07374.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:journals/jmlr/RossGB11,
  author    = {St{\'{e}}phane Ross and
               Geoffrey J. Gordon and
               Drew Bagnell},
  editor    = {Geoffrey J. Gordon and
               David B. Dunson and
               Miroslav Dud{\'{\i}}k},
  title     = {A Reduction of Imitation Learning and Structured Prediction to No-Regret
               Online Learning},
  booktitle = {Proceedings of the Fourteenth International Conference on Artificial
               Intelligence and Statistics, {AISTATS} 2011, Fort Lauderdale, USA,
               April 11-13, 2011},
  series    = {{JMLR} Proceedings},
  volume    = {15},
  pages     = {627--635},
  publisher = {JMLR.org},
  year      = {2011},
  url       = {http://proceedings.mlr.press/v15/ross11a/ross11a.pdf},
  timestamp = {Wed, 29 May 2019 08:41:48 +0200},
  biburl    = {https://dblp.org/rec/journals/jmlr/RossGB11.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{causal_confusion,
  author    = {Pim de Haan and
               Dinesh Jayaraman and
               Sergey Levine},
  editor    = {Hanna M. Wallach and
               Hugo Larochelle and
               Alina Beygelzimer and
               Florence d'Alch{\'{e}}{-}Buc and
               Emily B. Fox and
               Roman Garnett},
  title     = {Causal Confusion in Imitation Learning},
  booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
               on Neural Information Processing Systems 2019, NeurIPS 2019, 8-14
               December 2019, Vancouver, BC, Canada},
  pages     = {11693--11704},
  year      = {2019},
  url       = {http://papers.nips.cc/paper/9343-causal-confusion-in-imitation-learning},
  timestamp = {Fri, 06 Mar 2020 16:59:09 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/HaanJL19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{carla,
  author    = {Alexey Dosovitskiy and
               Germ{\'{a}}n Ros and
               Felipe Codevilla and
               Antonio L{\'{o}}pez and
               Vladlen Koltun},
  title     = {{CARLA:} An Open Urban Driving Simulator},
  booktitle = {1st Annual Conference on Robot Learning, CoRL 2017, Mountain View,
               California, USA, November 13-15, 2017, Proceedings},
  series    = {Proceedings of Machine Learning Research},
  volume    = {78},
  pages     = {1--16},
  publisher = {{PMLR}},
  year      = {2017},
  url       = {http://proceedings.mlr.press/v78/dosovitskiy17a.html},
  timestamp = {Wed, 03 Apr 2019 18:17:24 +0200},
  biburl    = {https://dblp.org/rec/conf/corl/DosovitskiyRCLK17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icra/KendallHJMRALBS19,
  author    = {Alex Kendall and
               Jeffrey Hawke and
               David Janz and
               Przemyslaw Mazur and
               Daniele Reda and
               John{-}Mark Allen and
               Vinh{-}Dieu Lam and
               Alex Bewley and
               Amar Shah},
  title     = {Learning to Drive in a Day},
  booktitle = {International Conference on Robotics and Automation, {ICRA} 2019,
               Montreal, QC, Canada, May 20-24, 2019},
  pages     = {8248--8254},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICRA.2019.8793742},
  doi       = {10.1109/ICRA.2019.8793742},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/KendallHJMRALBS19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{traffic_patterns,
  author    = {Hongyi Zhang and
               Andreas Geiger and
               Raquel Urtasun},
  title     = {Understanding High-Level Semantics by Modeling Traffic Patterns},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2013, Sydney,
               Australia, December 1-8, 2013},
  pages     = {3056--3063},
  publisher = {{IEEE} Computer Society},
  year      = {2013},
  url       = {https://doi.org/10.1109/ICCV.2013.379},
  doi       = {10.1109/ICCV.2013.379},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iccv/ZhangGU13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{wojek2011occlusion,
  author    = {Christian Wojek and
               Stefan Walk and
               Stefan Roth and
               Bernt Schiele},
  title     = {Monocular 3D scene understanding with explicit occlusion reasoning},
  booktitle = {The 24th {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2011, Colorado Springs, CO, USA, 20-25 June 2011},
  pages     = {1993--2000},
  publisher = {{IEEE} Computer Society},
  year      = {2011},
  url       = {https://doi.org/10.1109/CVPR.2011.5995547},
  doi       = {10.1109/CVPR.2011.5995547},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/WojekWRS11.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{wojek2013pami,
  author    = {Christian Wojek and
               Stefan Walk and
               Stefan Roth and
               Konrad Schindler and
               Bernt Schiele},
  title     = {Monocular Visual Scene Understanding: Understanding Multi-Object Traffic
               Scenes},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {35},
  number    = {4},
  pages     = {882--897},
  year      = {2013},
  url       = {https://doi.org/10.1109/TPAMI.2012.174},
  doi       = {10.1109/TPAMI.2012.174},
  timestamp = {Wed, 14 Nov 2018 10:51:10 +0100},
  biburl    = {https://dblp.org/rec/journals/pami/WojekWRSS13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{wang2019parametric,
  author    = {Ziyan Wang and
               Buyu Liu and
               Samuel Schulter and
               Manmohan Chandraker},
  title     = {A Parametric Top-View Representation of Complex Road Scenes},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {10325--10333},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Wang\_A\_Parametric\_Top-View\_Representation\_of\_Complex\_Road\_Scenes\_CVPR\_2019\_paper.html},
  doi       = {10.1109/CVPR.2019.01057},
  timestamp = {Mon, 20 Jan 2020 15:36:04 +0100},
  biburl    = {https://dblp.org/rec/conf/cvpr/WangLSC19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{doescomputervisionmatterforaction,
  author    = {Brady Zhou and
               Philipp Kr{\"{a}}henb{\"{u}}hl and
               Vladlen Koltun},
  title     = {Does computer vision matter for action?},
  journal   = {Sci. Robotics},
  volume    = {4},
  number    = {30},
  year      = {2019},
  url       = {https://doi.org/10.1126/scirobotics.aaw6661},
  doi       = {10.1126/scirobotics.aaw6661},
  timestamp = {Fri, 27 Mar 2020 08:33:42 +0100},
  biburl    = {https://dblp.org/rec/journals/scirobotics/ZhouKK19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/eccv/CodevillaLKD18,
  author    = {Felipe Codevilla and
               Antonio L{\'{o}}pez and
               Vladlen Koltun and
               Alexey Dosovitskiy},
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {On Offline Evaluation of Vision-Based Driving Models},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {XV}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11219},
  pages     = {246--262},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-01267-0\_15},
  doi       = {10.1007/978-3-030-01267-0\_15},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/CodevillaLKD18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{lidar_based_driving,
  author    = {Luca Caltagirone and
               Mauro Bellone and
               Lennart Svensson and
               Mattias Wahde},
  title     = {LIDAR-based driving path generation using fully convolutional neural
               networks},
  booktitle = {20th {IEEE} International Conference on Intelligent Transportation
               Systems, {ITSC} 2017, Yokohama, Japan, October 16-19, 2017},
  pages     = {1--6},
  publisher = {{IEEE}},
  year      = {2017},
  url       = {https://doi.org/10.1109/ITSC.2017.8317618},
  doi       = {10.1109/ITSC.2017.8317618},
  timestamp = {Wed, 16 Oct 2019 14:14:57 +0200},
  biburl    = {https://dblp.org/rec/conf/itsc/CaltagironeBSW17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iui/AhmedBSMSG20,
  author    = {Subeida Ahmed and
               Harshadha Balasubramanian and
               Simone Stumpf and
               Cecily Morrison and
               Abigail Sellen and
               Martin Grayson},
  editor    = {Fabio Patern{\`{o}} and
               Nuria Oliver and
               Cristina Conati and
               Lucio Davide Spano and
               Nava Tintarev},
  title     = {Investigating the intelligibility of a computer vision system for
               blind users},
  booktitle = {{IUI} '20: 25th International Conference on Intelligent User Interfaces,
               Cagliari, Italy, March 17-20, 2020},
  pages     = {419--429},
  publisher = {{ACM}},
  year      = {2020},
  url       = {https://doi.org/10.1145/3377325.3377508},
  doi       = {10.1145/3377325.3377508},
  timestamp = {Fri, 06 Mar 2020 14:10:34 +0100},
  biburl    = {https://dblp.org/rec/conf/iui/AhmedBSMSG20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{uncertainty_explanation,
  author    = {Kirill Bykov and
               Marina M.{-}C. H{\"{o}}hne and
               Klaus{-}Robert M{\"{u}}ller and
               Shinichi Nakajima and
               Marius Kloft},
  title     = {How Much Can {I} Trust You? - Quantifying Uncertainties in Explaining
               Neural Networks},
  journal   = {CoRR},
  volume    = {abs/2006.09000},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.09000},
  archivePrefix = {arXiv},
  eprint    = {2006.09000},
  timestamp = {Wed, 17 Jun 2020 14:28:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-09000.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{dashboard_design,
  author    = {Nikhil Gowda and
               Wendy Ju and
               Kirstin Kohler},
  editor    = {Linda Ng Boyle and
               Gary E. Burnett and
               Peter Fr{\"{o}}hlich and
               Shamsi T. Iqbal and
               Erika Miller and
               Yuqing Wu},
  title     = {Dashboard Design for an Autonomous Car},
  booktitle = {Adjunct Proceedings of the 6th International Conference on Automotive
               User Interfaces and Interactive Vehicular Applications, Seattle, WA,
               USA, September 17 - 19, 2014},
  pages     = {5:1--5:4},
  publisher = {{ACM}},
  year      = {2014},
  url       = {https://doi.org/10.1145/2667239.2667313},
  doi       = {10.1145/2667239.2667313},
  timestamp = {Tue, 06 Nov 2018 11:07:44 +0100},
  biburl    = {https://dblp.org/rec/conf/automotiveUI/GowdaJK14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{shariff2017psychological,
  title={Psychological roadblocks to the adoption of self-driving vehicles},
  author={Shariff, Azim and Bonnefon, Jean-Fran{\c{c}}ois and Rahwan, Iyad},
  journal={Nature Human Behaviour},
  volume={1},
  number={10},
  pages={694--696},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{koo2015did,
  title={Why did my car just do that? Explaining semi-autonomous driving actions to improve driver understanding, trust, and performance},
  author={Koo, Jeamin and Kwac, Jungsuk and Ju, Wendy and Steinert, Martin and Leifer, Larry and Nass, Clifford},
  journal={International Journal on Interactive Design and Manufacturing (IJIDeM)},
  volume={9},
  number={4},
  pages={269--275},
  year={2015},
  publisher={Springer}
}

@inproceedings{chauffeurnet,
  author    = {Mayank Bansal and
               Alex Krizhevsky and
               Abhijit S. Ogale},
  editor    = {Antonio Bicchi and
               Hadas Kress{-}Gazit and
               Seth Hutchinson},
  title     = {ChauffeurNet: Learning to Drive by Imitating the Best and Synthesizing
               the Worst},
  booktitle = {Robotics: Science and Systems XV, University of Freiburg, Freiburg
               im Breisgau, Germany, June 22-26, 2019},
  year      = {2019},
  url       = {https://doi.org/10.15607/RSS.2019.XV.031},
  doi       = {10.15607/RSS.2019.XV.031},
  timestamp = {Wed, 18 Sep 2019 11:00:19 +0200},
  biburl    = {https://dblp.org/rec/conf/rss/BansalKO19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{uncertainty_aware_short_term_motion_prediction,
  author    = {Nemanja Djuric and
               Vladan Radosavljevic and
               Henggang Cui and
               Thi Nguyen and
               Fang{-}Chieh Chou and
               Tsung{-}Han Lin and
               Nitin Singh and
               Jeff Schneider},
  title     = {Uncertainty-aware Short-term Motion Prediction of Traffic Actors for
               Autonomous Driving},
  booktitle = {{IEEE} Winter Conference on Applications of Computer Vision, {WACV}
               2020, Snowmass Village, CO, USA, March 1-5, 2020},
  pages     = {2084--2093},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/WACV45572.2020.9093332},
  doi       = {10.1109/WACV45572.2020.9093332},
  timestamp = {Mon, 18 May 2020 20:02:36 +0200},
  biburl    = {https://dblp.org/rec/conf/wacv/DjuricRCNCLSS20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{oliveira2020influence,
  title={The influence of system transparency on trust: Evaluating interfaces in a highly automated vehicle},
  author={Oliveira, Luis and Burns, Christopher and Luton, Jacob and Iyer, Sumeet and Birrell, Stewart},
  journal={Transportation Research Part F: Traffic Psychology and Behaviour},
  volume={72},
  pages={280--296},
  year={2020},
  publisher={Elsevier}
}

@article{riquelme2020explaining,
  title={Explaining VQA predictions using visual grounding and a knowledge base},
  author={Riquelme, Felipe and De Goyeneche, Alfredo and Zhang, Yundong and Niebles, Juan Carlos and Soto, Alvaro},
  journal={Image and Vision Computing},
  pages={103968},
  year={2020},
  publisher={Elsevier}
}

@article{attentional_bottleneck,
  author    = {Jinkyu Kim and
               Mayank Bansal},
  title     = {Attentional Bottleneck: Towards an Interpretable Deep Driving Network},
  journal   = {CoRR},
  volume    = {abs/2005.04298},
  year      = {2020},
  url       = {https://arxiv.org/abs/2005.04298},
  archivePrefix = {arXiv},
  eprint    = {2005.04298},
  timestamp = {Thu, 14 May 2020 16:56:02 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2005-04298.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{neural_motion_planner,
  author    = {Wenyuan Zeng and
               Wenjie Luo and
               Simon Suo and
               Abbas Sadat and
               Bin Yang and
               Sergio Casas and
               Raquel Urtasun},
  title     = {End-To-End Interpretable Neural Motion Planner},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {8660--8669},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Zeng\_End-To-End\_Interpretable\_Neural\_Motion\_Planner\_CVPR\_2019\_paper.html},
  doi       = {10.1109/CVPR.2019.00886},
  timestamp = {Fri, 17 Apr 2020 16:06:25 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/ZengLSSYCU19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{multipath,
  author    = {Yuning Chai and
               Benjamin Sapp and
               Mayank Bansal and
               Dragomir Anguelov},
  editor    = {Leslie Pack Kaelbling and
               Danica Kragic and
               Komei Sugiura},
  title     = {MultiPath: Multiple Probabilistic Anchor Trajectory Hypotheses for
               Behavior Prediction},
  booktitle = {3rd Annual Conference on Robot Learning, CoRL 2019, Osaka, Japan,
               October 30 - November 1, 2019, Proceedings},
  series    = {Proceedings of Machine Learning Research},
  volume    = {100},
  pages     = {86--99},
  publisher = {{PMLR}},
  year      = {2019},
  url       = {http://proceedings.mlr.press/v100/chai20a.html},
  timestamp = {Mon, 25 May 2020 15:01:26 +0200},
  biburl    = {https://dblp.org/rec/conf/corl/ChaiSBA19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{monocular_plan,
  author    = {Dequan Wang and
               Coline Devin and
               Qi{-}Zhi Cai and
               Philipp Kr{\"{a}}henb{\"{u}}hl and
               Trevor Darrell},
  title     = {Monocular Plan View Networks for Autonomous Driving},
  booktitle = {2019 {IEEE/RSJ} International Conference on Intelligent Robots and
               Systems, {IROS} 2019, Macau, SAR, China, November 3-8, 2019},
  pages     = {2876--2883},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/IROS40897.2019.8967897},
  doi       = {10.1109/IROS40897.2019.8967897},
  timestamp = {Fri, 31 Jan 2020 13:28:16 +0100},
  biburl    = {https://dblp.org/rec/conf/iros/WangDCKD19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{deconvnet,
  author    = {Matthew D. Zeiler and
               Rob Fergus},
  editor    = {David J. Fleet and
               Tom{\'{a}}s Pajdla and
               Bernt Schiele and
               Tinne Tuytelaars},
  title     = {Visualizing and Understanding Convolutional Networks},
  booktitle = {Computer Vision - {ECCV} 2014 - 13th European Conference, Zurich,
               Switzerland, September 6-12, 2014, Proceedings, Part {I}},
  series    = {Lecture Notes in Computer Science},
  volume    = {8689},
  pages     = {818--833},
  publisher = {Springer},
  year      = {2014},
  url       = {https://doi.org/10.1007/978-3-319-10590-1\_53},
  doi       = {10.1007/978-3-319-10590-1\_53},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/ZeilerF14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{deep_object_centric,
  author    = {Dequan Wang and
               Coline Devin and
               Qi{-}Zhi Cai and
               Fisher Yu and
               Trevor Darrell},
  title     = {Deep Object-Centric Policies for Autonomous Driving},
  booktitle = {International Conference on Robotics and Automation, {ICRA} 2019,
               Montreal, QC, Canada, May 20-24, 2019},
  pages     = {8853--8859},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICRA.2019.8794224},
  doi       = {10.1109/ICRA.2019.8794224},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/WangDCYD19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{grounding_visual_explanations,
  author    = {Lisa Anne Hendricks and
               Ronghang Hu and
               Trevor Darrell and
               Zeynep Akata},
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {Grounding Visual Explanations},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {II}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11206},
  pages     = {269--286},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-01216-8\_17},
  doi       = {10.1007/978-3-030-01216-8\_17},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/HendricksHDA18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{multimodal_explanations,
  author    = {Dong Huk Park and
               Lisa Anne Hendricks and
               Zeynep Akata and
               Anna Rohrbach and
               Bernt Schiele and
               Trevor Darrell and
               Marcus Rohrbach},
  title     = {Multimodal Explanations: Justifying Decisions and Pointing to the
               Evidence},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {8779--8788},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Park\_Multimodal\_Explanations\_Justifying\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPR.2018.00915},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/ParkHARSDR18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{explainable_object_induced,
  author    = {Yiran Xu and
               Xiaoyin Yang and
               Lihang Gong and
               Hsuan{-}Chu Lin and
               Tz{-}Ying Wu and
               Yunsheng Li and
               Nuno Vasconcelos},
  title     = {Explainable Object-induced Action Decision for Autonomous Vehicles},
  journal   = {CoRR},
  volume    = {abs/2003.09405},
  year      = {2020},
  url       = {https://arxiv.org/abs/2003.09405},
  archivePrefix = {arXiv},
  eprint    = {2003.09405},
  timestamp = {Tue, 24 Mar 2020 16:42:29 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2003-09405.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{latent_deep_rl,
  author    = {Jianyu Chen and
               Shengbo Eben Li and
               Masayoshi Tomizuka},
  title     = {Interpretable End-to-end Urban Autonomous Driving with Latent Deep
               Reinforcement Learning},
  journal   = {CoRR},
  volume    = {abs/2001.08726},
  year      = {2020},
  url       = {https://arxiv.org/abs/2001.08726},
  archivePrefix = {arXiv},
  eprint    = {2001.08726},
  timestamp = {Fri, 24 Jan 2020 15:00:57 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2001-08726.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{cumulative_prospect_theory,
  author    = {Liting Sun and
               Wei Zhan and
               Yeping Hu and
               Masayoshi Tomizuka},
  title     = {Interpretable Modelling of Driving Behaviors in Interactive Driving
               Scenarios based on Cumulative Prospect Theory},
  booktitle = {2019 {IEEE} Intelligent Transportation Systems Conference, {ITSC}
               2019, Auckland, New Zealand, October 27-30, 2019},
  pages     = {4329--4335},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ITSC.2019.8916944},
  doi       = {10.1109/ITSC.2019.8916944},
  timestamp = {Mon, 09 Dec 2019 13:26:04 +0100},
  biburl    = {https://dblp.org/rec/conf/itsc/SunZHT19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{fast_furious,
  author    = {Wenjie Luo and
               Bin Yang and
               Raquel Urtasun},
  title     = {Fast and Furious: Real Time End-to-End 3D Detection, Tracking and
               Motion Forecasting With a Single Convolutional Net},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {3569--3577},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Luo\_Fast\_and\_Furious\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPR.2018.00376},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/LuoYU18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{intentnet,
  author    = {Sergio Casas and
               Wenjie Luo and
               Raquel Urtasun},
  title     = {IntentNet: Learning to Predict Intention from Raw Sensor Data},
  booktitle = {2nd Annual Conference on Robot Learning, CoRL 2018, Z{\"{u}}rich,
               Switzerland, 29-31 October 2018, Proceedings},
  series    = {Proceedings of Machine Learning Research},
  volume    = {87},
  pages     = {947--956},
  publisher = {{PMLR}},
  year      = {2018},
  url       = {http://proceedings.mlr.press/v87/casas18a.html},
  timestamp = {Fri, 17 Apr 2020 16:06:29 +0200},
  biburl    = {https://dblp.org/rec/conf/corl/CasasLU18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{felleman1991distributed,
  title={Distributed hierarchical processing in the primate cerebral cortex.},
  author={Felleman, Daniel J and Van Essen, David C},
  journal={Cerebral cortex (New York, NY: 1991)},
  volume={1},
  number={1},
  pages={1--47},
  year={1991}
}

@book{kandel2000principles,
  title={Principles of neural science},
  author={Kandel, Eric R and Schwartz, James H and Jessell, Thomas M and Department of Biochemistry and Molecular Biophysics Thomas Jessell and Siegelbaum, Steven and Hudspeth, AJ},
  volume={4},
  year={2000},
  publisher={McGraw-hill New York}
}

@article{bertenthal1996origins,
  title={Origins and early development of perception, action, and representation},
  author={Bertenthal, Bennett I},
  journal={Annual review of psychology},
  volume={47},
  number={1},
  pages={431--459},
  year={1996},
  publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
}

@inproceedings{mataric2000sensory,
  title={Sensory-motor primitives as a basis for imitation: Linking perception to action and biology to robotics},
  author={Mataric, Maja J},
  booktitle={Imitation in Animals and Artifacts},
  year={2000},
  organization={Citeseer}
}

@article{flash2005motor,
  title={Motor primitives in vertebrates and invertebrates},
  author={Flash, Tamar and Hochner, Binyamin},
  journal={Current opinion in neurobiology},
  volume={15},
  number={6},
  pages={660--666},
  year={2005},
  publisher={Elsevier}
}

@article{hart2010neural,
  title={A neural basis for motor primitives in the spinal cord},
  author={Hart, Corey B and Giszter, Simon F},
  journal={Journal of Neuroscience},
  volume={30},
  number={4},
  pages={1322--1336},
  year={2010},
  publisher={Soc Neuroscience}
}

@inproceedings{driving_policy_transfer,
  author    = {Matthias M{\"{u}}ller and
               Alexey Dosovitskiy and
               Bernard Ghanem and
               Vladlen Koltun},
  title     = {Driving Policy Transfer via Modularity and Abstraction},
  booktitle = {2nd Annual Conference on Robot Learning, CoRL 2018, Z{\"{u}}rich,
               Switzerland, 29-31 October 2018, Proceedings},
  series    = {Proceedings of Machine Learning Research},
  volume    = {87},
  pages     = {1--15},
  publisher = {{PMLR}},
  year      = {2018},
  url       = {http://proceedings.mlr.press/v87/mueller18a.html},
  timestamp = {Wed, 19 Feb 2020 17:10:31 +0100},
  biburl    = {https://dblp.org/rec/conf/corl/MuellerDGK18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{accident_explanation_ability,
  author    = {Zhihao Li and
               Toshiyuki Motoyoshi and
               Kazuma Sasaki and
               Tetsuya Ogata and
               Shigeki Sugano},
  title     = {Rethinking Self-driving: Multi-task Knowledge for Better Generalization
               and Accident Explanation Ability},
  journal   = {CoRR},
  volume    = {abs/1809.11100},
  year      = {2018},
  url       = {http://arxiv.org/abs/1809.11100},
  archivePrefix = {arXiv},
  eprint    = {1809.11100},
  timestamp = {Fri, 05 Oct 2018 11:34:52 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1809-11100.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{visualbackprop,
  author    = {Mariusz Bojarski and
               Anna Choromanska and
               Krzysztof Choromanski and
               Bernhard Firner and
               Larry J. Ackel and
               Urs Muller and
               Philip Yeres and
               Karol Zieba},
  title     = {VisualBackProp: Efficient Visualization of CNNs for Autonomous Driving},
  booktitle = {2018 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2018, Brisbane, Australia, May 21-25, 2018},
  pages     = {1--8},
  publisher = {{IEEE}},
  year      = {2018},
  url       = {https://doi.org/10.1109/ICRA.2018.8461053},
  doi       = {10.1109/ICRA.2018.8461053},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/BojarskiCCFAMYZ18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{explaining_pilotnet,
  author    = {Mariusz Bojarski and
               Philip Yeres and
               Anna Choromanska and
               Krzysztof Choromanski and
               Bernhard Firner and
               Lawrence D. Jackel and
               Urs Muller},
  title     = {Explaining How a Deep Neural Network Trained with End-to-End Learning
               Steers a Car},
  journal   = {CoRR},
  volume    = {abs/1704.07911},
  year      = {2017},
  url       = {http://arxiv.org/abs/1704.07911},
  archivePrefix = {arXiv},
  eprint    = {1704.07911},
  timestamp = {Mon, 13 Aug 2018 16:46:51 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/BojarskiYCCFJM17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{against_direct_perception,
  title={Against direct perception},
  author={Ullman, Shimon},
  year={1980}
}

@article{gradcam,
  author    = {Ramprasaath R. Selvaraju and
               Michael Cogswell and
               Abhishek Das and
               Ramakrishna Vedantam and
               Devi Parikh and
               Dhruv Batra},
  title     = {Grad-CAM: Visual Explanations from Deep Networks via Gradient-Based
               Localization},
  journal   = {Int. J. Comput. Vis.},
  volume    = {128},
  number    = {2},
  pages     = {336--359},
  year      = {2020},
  url       = {https://doi.org/10.1007/s11263-019-01228-7},
  doi       = {10.1007/s11263-019-01228-7},
  timestamp = {Fri, 13 Mar 2020 10:58:48 +0100},
  biburl    = {https://dblp.org/rec/journals/ijcv/SelvarajuCDVPB20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{xai_human_agent,
  author    = {Avi Rosenfeld and
               Ariella Richardson},
  editor    = {Amal El Fallah Seghrouchni and
               Gita Sukthankar and
               Bo An and
               Neil Yorke{-}Smith},
  title     = {Why, Who, What, When and How about Explainability in Human-Agent Systems},
  booktitle = {Proceedings of the 19th International Conference on Autonomous Agents
               and Multiagent Systems, {AAMAS} '20, Auckland, New Zealand, May 9-13,
               2020},
  pages     = {2161--2164},
  publisher = {International Foundation for Autonomous Agents and Multiagent Systems},
  year      = {2020},
  url       = {https://dl.acm.org/doi/abs/10.5555/3398761.3399110},
  timestamp = {Fri, 05 Jun 2020 12:49:45 +0200},
  biburl    = {https://dblp.org/rec/conf/atal/RosenfeldR20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{cam,
  author    = {Bolei Zhou and
               Aditya Khosla and
               {\`{A}}gata Lapedriza and
               Aude Oliva and
               Antonio Torralba},
  title     = {Learning Deep Features for Discriminative Localization},
  booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016},
  pages     = {2921--2929},
  publisher = {{IEEE} Computer Society},
  year      = {2016},
  url       = {https://doi.org/10.1109/CVPR.2016.319},
  doi       = {10.1109/CVPR.2016.319},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/ZhouKLOT16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{attack_explain,
  title={Attack to Explain Deep Representation},
  author={Jalwana, Mohammad AAK and Akhtar, Naveed and Bennamoun, Mohammed and Mian, Ajmal},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9543--9552},
  year={2020}
}

@inproceedings{generating_visual_explanations,
  author    = {Lisa Anne Hendricks and
               Zeynep Akata and
               Marcus Rohrbach and
               Jeff Donahue and
               Bernt Schiele and
               Trevor Darrell},
  editor    = {Bastian Leibe and
               Jiri Matas and
               Nicu Sebe and
               Max Welling},
  title     = {Generating Visual Explanations},
  booktitle = {Computer Vision - {ECCV} 2016 - 14th European Conference, Amsterdam,
               The Netherlands, October 11-14, 2016, Proceedings, Part {IV}},
  series    = {Lecture Notes in Computer Science},
  volume    = {9908},
  pages     = {3--19},
  publisher = {Springer},
  year      = {2016},
  url       = {https://doi.org/10.1007/978-3-319-46493-0\_1},
  doi       = {10.1007/978-3-319-46493-0\_1},
  timestamp = {Wed, 25 Sep 2019 18:11:12 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/HendricksARDSD16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{xai_field_guide,
  author    = {Ning Xie and
               Gabrielle Ras and
               Marcel van Gerven and
               Derek Doran},
  title     = {Explainable Deep Learning: {A} Field Guide for the Uninitiated},
  journal   = {CoRR},
  volume    = {abs/2004.14545},
  year      = {2020},
  url       = {https://arxiv.org/abs/2004.14545},
  archivePrefix = {arXiv},
  eprint    = {2004.14545},
  timestamp = {Sun, 03 May 2020 17:39:04 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2004-14545.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{xai_systematic_review,
  author    = {Giulia Vilone and
               Luca Longo},
  title     = {Explainable Artificial Intelligence: a Systematic Review},
  journal   = {CoRR},
  volume    = {abs/2006.00093},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.00093},
  archivePrefix = {arXiv},
  eprint    = {2006.00093},
  timestamp = {Mon, 08 Jun 2020 15:48:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-00093.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{xai_causal,
  author    = {Raha Moraffah and
               Mansooreh Karami and
               Ruocheng Guo and
               Adrienne Raglin and
               Huan Liu},
  title     = {Causal Interpretability for Machine Learning - Problems, Methods and
               Evaluation},
  journal   = {{SIGKDD} Explorations},
  volume    = {22},
  number    = {1},
  pages     = {18--33},
  year      = {2020},
  url       = {https://doi.org/10.1145/3400051.3400058},
  doi       = {10.1145/3400051.3400058},
  timestamp = {Wed, 27 May 2020 14:16:43 +0200},
  biburl    = {https://dblp.org/rec/journals/sigkdd/MoraffahKGRL20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{xai_peeking_inside_black_box,
  author    = {Amina Adadi and
               Mohammed Berrada},
  title     = {Peeking Inside the Black-Box: {A} Survey on Explainable Artificial
               Intelligence {(XAI)}},
  journal   = {{IEEE} Access},
  volume    = {6},
  pages     = {52138--52160},
  year      = {2018},
  url       = {https://doi.org/10.1109/ACCESS.2018.2870052},
  doi       = {10.1109/ACCESS.2018.2870052},
  timestamp = {Mon, 16 Sep 2019 14:46:21 +0200},
  biburl    = {https://dblp.org/rec/journals/access/AdadiB18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{shap_tree,
  title={From local explanations to global understanding with explainable AI for trees},
  author={Lundberg, Scott M and Erion, Gabriel and Chen, Hugh and DeGrave, Alex and Prutkin, Jordan M and Nair, Bala and Katz, Ronit and Himmelfarb, Jonathan and Bansal, Nisha and Lee, Su-In},
  journal={Nature machine intelligence},
  volume={2},
  number={1},
  pages={2522--5839},
  year={2020}
}

@inproceedings{meaningful_perturbations,
  author    = {Ruth C. Fong and
               Andrea Vedaldi},
  title     = {Interpretable Explanations of Black Boxes by Meaningful Perturbation},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2017, Venice,
               Italy, October 22-29, 2017},
  pages     = {3449--3457},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/ICCV.2017.371},
  doi       = {10.1109/ICCV.2017.371},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iccv/FongV17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{guided_backprop,
  author    = {Aravindh Mahendran and
               Andrea Vedaldi},
  editor    = {Bastian Leibe and
               Jiri Matas and
               Nicu Sebe and
               Max Welling},
  title     = {Salient Deconvolutional Networks},
  booktitle = {Computer Vision - {ECCV} 2016 - 14th European Conference, Amsterdam,
               The Netherlands, October 11-14, 2016, Proceedings, Part {VI}},
  series    = {Lecture Notes in Computer Science},
  volume    = {9910},
  pages     = {120--135},
  publisher = {Springer},
  year      = {2016},
  url       = {https://doi.org/10.1007/978-3-319-46466-4\_8},
  doi       = {10.1007/978-3-319-46466-4\_8},
  timestamp = {Wed, 25 Sep 2019 18:11:13 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/MahendranV16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{lrp,
  title={On pixel-wise explanations for non-linear classifier decisions by layer-wise relevance propagation},
  author={Bach, Sebastian and Binder, Alexander and Montavon, Gr{\'e}goire and Klauschen, Frederick and M{\"u}ller, Klaus-Robert and Samek, Wojciech},
  journal={PloS one},
  volume={10},
  number={7},
  pages={e0130140},
  year={2015},
  publisher={Public Library of Science}
}

@inproceedings{object_detectors_emerge_in_deep_scene,
  author    = {Bolei Zhou and
               Aditya Khosla and
               {\`{A}}gata Lapedriza and
               Aude Oliva and
               Antonio Torralba},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Object Detectors Emerge in Deep Scene CNNs},
  booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
               San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
  year      = {2015},
  url       = {http://arxiv.org/abs/1412.6856},
  timestamp = {Wed, 17 Jul 2019 10:40:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/ZhouKLOT14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{deeplift,
  author    = {Avanti Shrikumar and
               Peyton Greenside and
               Anshul Kundaje},
  editor    = {Doina Precup and
               Yee Whye Teh},
  title     = {Learning Important Features Through Propagating Activation Differences},
  booktitle = {Proceedings of the 34th International Conference on Machine Learning,
               {ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
  series    = {Proceedings of Machine Learning Research},
  volume    = {70},
  pages     = {3145--3153},
  publisher = {{PMLR}},
  year      = {2017},
  url       = {http://proceedings.mlr.press/v70/shrikumar17a.html},
  timestamp = {Wed, 29 May 2019 08:41:45 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/ShrikumarGK17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{integrated_gradients,
  author    = {Mukund Sundararajan and
               Ankur Taly and
               Qiqi Yan},
  editor    = {Doina Precup and
               Yee Whye Teh},
  title     = {Axiomatic Attribution for Deep Networks},
  booktitle = {Proceedings of the 34th International Conference on Machine Learning,
               {ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
  series    = {Proceedings of Machine Learning Research},
  volume    = {70},
  pages     = {3319--3328},
  publisher = {{PMLR}},
  year      = {2017},
  url       = {http://proceedings.mlr.press/v70/sundararajan17a.html},
  timestamp = {Wed, 29 May 2019 08:41:45 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/SundararajanTY17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{deepred,
  author    = {Jan Ruben Zilke and
               Eneldo Loza Menc{\'{\i}}a and
               Frederik Janssen},
  editor    = {Toon Calders and
               Michelangelo Ceci and
               Donato Malerba},
  title     = {DeepRED - Rule Extraction from Deep Neural Networks},
  booktitle = {Discovery Science - 19th International Conference, {DS} 2016, Bari,
               Italy, October 19-21, 2016, Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {9956},
  pages     = {457--473},
  year      = {2016},
  url       = {https://doi.org/10.1007/978-3-319-46307-0\_29},
  doi       = {10.1007/978-3-319-46307-0\_29},
  timestamp = {Tue, 14 May 2019 10:00:46 +0200},
  biburl    = {https://dblp.org/rec/conf/dis/ZilkeMJ16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{self_attention_temporal_reasoning,
  author    = {Yi{-}Chieh Liu and
               Yung{-}An Hsieh and
               Min{-}Hung Chen and
               Chao{-}Han Huck Yang and
               Jesper Tegn{\'{e}}r and
               Yi{-}Chang James Tsai},
  title     = {Interpretable Self-Attention Temporal Reasoning for Driving Behavior
               Understanding},
  journal   = {CoRR},
  volume    = {abs/1911.02172},
  year      = {2019},
  url       = {http://arxiv.org/abs/1911.02172},
  archivePrefix = {arXiv},
  eprint    = {1911.02172},
  timestamp = {Mon, 11 Nov 2019 18:38:09 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1911-02172.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{situational_driving,
  title={Learning Situational Driving},
  author={Ohn-Bar, Eshed and Prakash, Aditya and Behl, Aseem and Chitta, Kashyap and Geiger, Andreas},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11296--11305},
  year={2020}
}

@inproceedings{mtp,
  author    = {Henggang Cui and
               Vladan Radosavljevic and
               Fang{-}Chieh Chou and
               Tsung{-}Han Lin and
               Thi Nguyen and
               Tzu{-}Kuo Huang and
               Jeff Schneider and
               Nemanja Djuric},
  title     = {Multimodal Trajectory Predictions for Autonomous Driving using Deep
               Convolutional Networks},
  booktitle = {International Conference on Robotics and Automation, {ICRA} 2019,
               Montreal, QC, Canada, May 20-24, 2019},
  pages     = {2090--2096},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICRA.2019.8793868},
  doi       = {10.1109/ICRA.2019.8793868},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/CuiRCLNHSD19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{multiple_futures,
  author    = {Yichuan Charlie Tang and
               Ruslan Salakhutdinov},
  editor    = {Hanna M. Wallach and
               Hugo Larochelle and
               Alina Beygelzimer and
               Florence d'Alch{\'{e}}{-}Buc and
               Emily B. Fox and
               Roman Garnett},
  title     = {Multiple Futures Prediction},
  booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
               on Neural Information Processing Systems 2019, NeurIPS 2019, 8-14
               December 2019, Vancouver, BC, Canada},
  pages     = {15398--15408},
  year      = {2019},
  url       = {http://papers.nips.cc/paper/9676-multiple-futures-prediction},
  timestamp = {Fri, 06 Mar 2020 17:00:10 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/TangS19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{covernet,
  author    = {Tung Phan{-}Minh and
               Elena Corina Grigore and
               Freddy A. Boulton and
               Oscar Beijbom and
               Eric M. Wolff},
  title     = {CoverNet: Multimodal Behavior Prediction using Trajectory Sets},
  journal   = {CoRR},
  volume    = {abs/1911.10298},
  year      = {2019},
  url       = {http://arxiv.org/abs/1911.10298},
  archivePrefix = {arXiv},
  eprint    = {1911.10298},
  timestamp = {Tue, 03 Dec 2019 14:15:54 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1911-10298.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{garden_of_forking_path,
  author    = {Junwei Liang and
               Lu Jiang and
               Kevin P. Murphy and
               Ting Yu and
               Alexander G. Hauptmann},
  title     = {The Garden of Forking Paths: Towards Multi-Future Trajectory Prediction},
  journal   = {CoRR},
  volume    = {abs/1912.06445},
  year      = {2019},
  url       = {http://arxiv.org/abs/1912.06445},
  archivePrefix = {arXiv},
  eprint    = {1912.06445},
  timestamp = {Thu, 02 Jan 2020 18:08:18 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1912-06445.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{mantra,
  author    = {Francesco Marchetti and
               Federico Becattini and
               Lorenzo Seidenari and
               Alberto Del Bimbo},
  title     = {{MANTRA:} Memory Augmented Networks for Multiple Trajectory Prediction},
  journal   = {CoRR},
  volume    = {abs/2006.03340},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.03340},
  archivePrefix = {arXiv},
  eprint    = {2006.03340},
  timestamp = {Mon, 08 Jun 2020 15:48:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-03340.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{human_like_driving,
  title={Learning Accurate and Human-Like Driving using Semantic Maps and Attention},
  author={Hecker, Simon and Dai, Dengxin and Liniger, Alexander and Van Gool, Luc},
  journal={arXiv preprint arXiv:2007.07218},
  year={2020}
}

@inproceedings{human_like_driving_simulator,
  author    = {Talal Al{-}Shihabi and
               Ronald R. Mourant},
  editor    = {Elisabeth Andr{\'{e}} and
               Sandip Sen and
               Claude Frasson and
               J{\"{o}}rg P. M{\"{u}}ller},
  title     = {A framework for modeling human-like driving behaviors for autonomous
               vehicles in driving simulators},
  booktitle = {Proceedings of the Fifth International Conference on Autonomous Agents,
               {AGENTS} 2001, Montreal, Canada, May 28 - June 1, 2001},
  pages     = {286--291},
  publisher = {{ACM}},
  year      = {2001},
  url       = {https://doi.org/10.1145/375735.376310},
  doi       = {10.1145/375735.376310},
  timestamp = {Tue, 06 Nov 2018 11:07:01 +0100},
  biburl    = {https://dblp.org/rec/conf/agents/Al-ShihabiM01.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{al2003toward,
  title={Toward more realistic driving behavior models for autonomous vehicles in driving simulators},
  author={Al-Shihabi, Talal and Mourant, Ronald R},
  journal={Transportation Research Record},
  volume={1843},
  number={1},
  pages={41--49},
  year={2003},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{gu2017human,
  title={Human-like motion planning model for driving in signalized intersections},
  author={Gu, Yanlei and Hashimoto, Yoriyoshi and Hsu, Li-Ta and Iryo-Asano, Miho and Kamijo, Shunsuke},
  journal={IATSS research},
  volume={41},
  number={3},
  pages={129--139},
  year={2017},
  publisher={Elsevier}
}

@inproceedings{drive_without_real_world_labels,
  author    = {Alex Bewley and
               Jessica Rigley and
               Yuxuan Liu and
               Jeffrey Hawke and
               Richard Shen and
               Vinh{-}Dieu Lam and
               Alex Kendall},
  title     = {Learning to Drive from Simulation without Real World Labels},
  booktitle = {International Conference on Robotics and Automation, {ICRA} 2019,
               Montreal, QC, Canada, May 20-24, 2019},
  pages     = {4818--4824},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICRA.2019.8793668},
  doi       = {10.1109/ICRA.2019.8793668},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/BewleyRLHSLK19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{grounding_human_vehicle_advice,
  author    = {Jinkyu Kim and
               Teruhisa Misu and
               Yi{-}Ting Chen and
               Ashish Tawari and
               John F. Canny},
  title     = {Grounding Human-To-Vehicle Advice for Self-Driving Vehicles},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {10591--10599},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Kim\_Grounding\_Human-To-Vehicle\_Advice\_for\_Self-Driving\_Vehicles\_CVPR\_2019\_paper.html},
  doi       = {10.1109/CVPR.2019.01084},
  timestamp = {Mon, 20 Jan 2020 15:36:04 +0100},
  biburl    = {https://dblp.org/rec/conf/cvpr/KimMCTC19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{di2020survey,
  title={A Survey on Autonomous Vehicle Control in the Era of Mixed-Autonomy: From Physics-Based to AI-Guided Driving Policy Learning},
  author={Di, Xuan and Shi, Rongye},
  journal={arXiv preprint arXiv:2007.05156},
  year={2020}
}

@article{geiger,
  author    = {Joel Janai and
               Fatma G{\"{u}}ney and
               Aseem Behl and
               Andreas Geiger},
  title     = {Computer Vision for Autonomous Vehicles: Problems, Datasets and State-of-the-Art},
  journal   = {CoRR},
  volume    = {abs/1704.05519},
  year      = {2017},
  url       = {http://arxiv.org/abs/1704.05519},
  archivePrefix = {arXiv},
  eprint    = {1704.05519},
  timestamp = {Mon, 13 Aug 2018 16:47:19 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/JanaiGBG17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{imitation_overview,
  title={Learning to drive by imitation: an overview of deep behavior cloning methods},
  author={Ly, Abdoulaye Oumar and Akhloufi, Moulay A},
  journal={IEEE Transactions on Intelligent Vehicles},
  year={2020},
  publisher={IEEE}
}

@inproceedings{vae_driving,
  author    = {Alexander Amini and
               Wilko Schwarting and
               Guy Rosman and
               Brandon Araki and
               Sertac Karaman and
               Daniela Rus},
  title     = {Variational Autoencoder for End-to-End Control of Autonomous Driving
               with Novelty Detection and Training De-biasing},
  booktitle = {2018 {IEEE/RSJ} International Conference on Intelligent Robots and
               Systems, {IROS} 2018, Madrid, Spain, October 1-5, 2018},
  pages     = {568--575},
  publisher = {{IEEE}},
  year      = {2018},
  url       = {https://doi.org/10.1109/IROS.2018.8594386},
  doi       = {10.1109/IROS.2018.8594386},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iros/AminiSRAKR18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{vae,
  author    = {Diederik P. Kingma and
               Max Welling},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Auto-Encoding Variational Bayes},
  booktitle = {2nd International Conference on Learning Representations, {ICLR} 2014,
               Banff, AB, Canada, April 14-16, 2014, Conference Track Proceedings},
  year      = {2014},
  url       = {http://arxiv.org/abs/1312.6114},
  timestamp = {Thu, 04 Apr 2019 13:20:07 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/KingmaW13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{approximate_inference_generative_models,
  author    = {Danilo Jimenez Rezende and
               Shakir Mohamed and
               Daan Wierstra},
  title     = {Stochastic Backpropagation and Approximate Inference in Deep Generative
               Models},
  booktitle = {Proceedings of the 31th International Conference on Machine Learning,
               {ICML} 2014, Beijing, China, 21-26 June 2014},
  series    = {{JMLR} Workshop and Conference Proceedings},
  volume    = {32},
  pages     = {1278--1286},
  publisher = {JMLR.org},
  year      = {2014},
  url       = {http://proceedings.mlr.press/v32/rezende14.html},
  timestamp = {Wed, 29 May 2019 08:41:45 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/RezendeMW14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{vae_images,
  author    = {Yunchen Pu and
               Zhe Gan and
               Ricardo Henao and
               Xin Yuan and
               Chunyuan Li and
               Andrew Stevens and
               Lawrence Carin},
  editor    = {Daniel D. Lee and
               Masashi Sugiyama and
               Ulrike von Luxburg and
               Isabelle Guyon and
               Roman Garnett},
  title     = {Variational Autoencoder for Deep Learning of Images, Labels and Captions},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {2352--2360},
  year      = {2016},
  url       = {http://papers.nips.cc/paper/6528-variational-autoencoder-for-deep-learning-of-images-labels-and-captions},
  timestamp = {Fri, 06 Mar 2020 17:00:31 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/PuGHYLSC16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{variational_navigation_localization,
  author    = {Alexander Amini and
               Guy Rosman and
               Sertac Karaman and
               Daniela Rus},
  title     = {Variational End-to-End Navigation and Localization},
  booktitle = {International Conference on Robotics and Automation, {ICRA} 2019,
               Montreal, QC, Canada, May 20-24, 2019},
  pages     = {8958--8964},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICRA.2019.8793579},
  doi       = {10.1109/ICRA.2019.8793579},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/AminiRKR19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@book{pearl_causality,
  title={Causality},
  author={Pearl, Judea},
  year={2009},
  publisher={Cambridge university press}
}

@article{causal_learning_autoencoded_activations,
  author    = {Michael Harradon and
               Jeff Druce and
               Brian E. Ruttenberg},
  title     = {Causal Learning and Explanation of Deep Neural Networks via Autoencoded
               Activations},
  journal   = {CoRR},
  volume    = {abs/1802.00541},
  year      = {2018},
  url       = {http://arxiv.org/abs/1802.00541},
  archivePrefix = {arXiv},
  eprint    = {1802.00541},
  timestamp = {Mon, 13 Aug 2018 16:49:12 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1802-00541.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{explaining_deep_causal_inference,
  author    = {Tanmayee Narendra and
               Anush Sankaran and
               Deepak Vijaykeerthy and
               Senthil Mani},
  title     = {Explaining Deep Learning Models using Causal Inference},
  journal   = {CoRR},
  volume    = {abs/1811.04376},
  year      = {2018},
  url       = {http://arxiv.org/abs/1811.04376},
  archivePrefix = {arXiv},
  eprint    = {1811.04376},
  timestamp = {Fri, 23 Nov 2018 12:43:51 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1811-04376.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{explaining_classifiers_counterfactual_explanations,
  author    = {Ramaravind Kommiya Mothilal and
               Amit Sharma and
               Chenhao Tan},
  editor    = {Mireille Hildebrandt and
               Carlos Castillo and
               Elisa Celis and
               Salvatore Ruggieri and
               Linnet Taylor and
               Gabriela Zanfir{-}Fortuna},
  title     = {Explaining machine learning classifiers through diverse counterfactual
               explanations},
  booktitle = {FAT* '20: Conference on Fairness, Accountability, and Transparency,
               Barcelona, Spain, January 27-30, 2020},
  pages     = {607--617},
  publisher = {{ACM}},
  year      = {2020},
  url       = {https://doi.org/10.1145/3351095.3372850},
  doi       = {10.1145/3351095.3372850},
  timestamp = {Thu, 26 Mar 2020 12:29:40 +0100},
  biburl    = {https://dblp.org/rec/conf/fat/MothilalST20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{counterfactual_visual_explanations,
  author    = {Yash Goyal and
               Ziyan Wu and
               Jan Ernst and
               Dhruv Batra and
               Devi Parikh and
               Stefan Lee},
  editor    = {Kamalika Chaudhuri and
               Ruslan Salakhutdinov},
  title     = {Counterfactual Visual Explanations},
  booktitle = {Proceedings of the 36th International Conference on Machine Learning,
               {ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
  series    = {Proceedings of Machine Learning Research},
  volume    = {97},
  pages     = {2376--2384},
  publisher = {{PMLR}},
  year      = {2019},
  url       = {http://proceedings.mlr.press/v97/goyal19a.html},
  timestamp = {Tue, 11 Jun 2019 15:37:38 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/GoyalWEBPL19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{nn_attributions_causal,
  author    = {Aditya Chattopadhyay and
               Piyushi Manupriya and
               Anirban Sarkar and
               Vineeth N. Balasubramanian},
  editor    = {Kamalika Chaudhuri and
               Ruslan Salakhutdinov},
  title     = {Neural Network Attributions: {A} Causal Perspective},
  booktitle = {Proceedings of the 36th International Conference on Machine Learning,
               {ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
  series    = {Proceedings of Machine Learning Research},
  volume    = {97},
  pages     = {981--990},
  publisher = {{PMLR}},
  year      = {2019},
  url       = {http://proceedings.mlr.press/v97/chattopadhyay19a.html},
  timestamp = {Tue, 11 Jun 2019 15:37:38 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/ChattopadhyayMS19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{counterfactuals_generative_models,
  author    = {Michel Besserve and
               Arash Mehrjou and
               R{\'{e}}my Sun and
               Bernhard Sch{\"{o}}lkopf},
  title     = {Counterfactuals uncover the modular structure of deep generative models},
  booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
               Addis Ababa, Ethiopia, April 26-30, 2020},
  publisher = {OpenReview.net},
  year      = {2020},
  url       = {https://openreview.net/forum?id=SJxDDpEKvH},
  timestamp = {Thu, 07 May 2020 17:11:47 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/BesserveMSS20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{rl_causal_lens,
  author    = {Prashan Madumal and
               Tim Miller and
               Liz Sonenberg and
               Frank Vetere},
  title     = {Explainable Reinforcement Learning through a Causal Lens},
  booktitle = {The Thirty-Fourth {AAAI} Conference on Artificial Intelligence, {AAAI}
               2020, The Thirty-Second Innovative Applications of Artificial Intelligence
               Conference, {IAAI} 2020, The Tenth {AAAI} Symposium on Educational
               Advances in Artificial Intelligence, {EAAI} 2020, New York, NY, USA,
               February 7-12, 2020},
  pages     = {2493--2500},
  publisher = {{AAAI} Press},
  year      = {2020},
  url       = {https://aaai.org/ojs/index.php/AAAI/article/view/5631},
  timestamp = {Fri, 05 Jun 2020 09:50:08 +0200},
  biburl    = {https://dblp.org/rec/conf/aaai/Madumal0SV20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1711-00399,
  author    = {Sandra Wachter and
               Brent D. Mittelstadt and
               Chris Russell},
  title     = {Counterfactual Explanations without Opening the Black Box: Automated
               Decisions and the {GDPR}},
  journal   = {CoRR},
  volume    = {abs/1711.00399},
  year      = {2017},
  url       = {http://arxiv.org/abs/1711.00399},
  archivePrefix = {arXiv},
  eprint    = {1711.00399},
  timestamp = {Wed, 23 Jan 2019 13:31:00 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1711-00399.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{counterfactual_black_box_gdpr,
  author    = {Sandra Wachter and
               Brent D. Mittelstadt and
               Chris Russell},
  title     = {Counterfactual Explanations without Opening the Black Box: Automated
               Decisions and the {GDPR}},
  journal   = {CoRR},
  volume    = {abs/1711.00399},
  year      = {2017},
  url       = {http://arxiv.org/abs/1711.00399},
  archivePrefix = {arXiv},
  eprint    = {1711.00399},
  timestamp = {Wed, 23 Jan 2019 13:31:00 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1711-00399.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{goyal_cace,
  author    = {Yash Goyal and
               Uri Shalit and
               Been Kim},
  title     = {Explaining Classifiers with Causal Concept Effect (CaCE)},
  journal   = {CoRR},
  volume    = {abs/1907.07165},
  year      = {2019},
  url       = {http://arxiv.org/abs/1907.07165},
  archivePrefix = {arXiv},
  eprint    = {1907.07165},
  timestamp = {Tue, 23 Jul 2019 10:54:22 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1907-07165.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{counterfactual_videos,
  author    = {Atsushi Kanehira and
               Kentaro Takemoto and
               Sho Inayoshi and
               Tatsuya Harada},
  title     = {Multimodal Explanations by Predicting Counterfactuality in Videos},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {8594--8602},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Kanehira\_Multimodal\_Explanations\_by\_Predicting\_Counterfactuality\_in\_Videos\_CVPR\_2019\_paper.html},
  doi       = {10.1109/CVPR.2019.00879},
  timestamp = {Mon, 20 Jan 2020 15:36:04 +0100},
  biburl    = {https://dblp.org/rec/conf/cvpr/KanehiraTIH19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{generative_causal_explanations_black_box,
  author    = {Matthew R. O'Shaughnessy and
               Gregory Canal and
               Marissa Connor and
               Mark A. Davenport and
               Christopher Rozell},
  title     = {Generative causal explanations of black-box classifiers},
  journal   = {CoRR},
  volume    = {abs/2006.13913},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.13913},
  archivePrefix = {arXiv},
  eprint    = {2006.13913},
  timestamp = {Wed, 01 Jul 2020 15:21:23 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-13913.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{show_attend_tell,
  author    = {Kelvin Xu and
               Jimmy Ba and
               Ryan Kiros and
               Kyunghyun Cho and
               Aaron C. Courville and
               Ruslan Salakhutdinov and
               Richard S. Zemel and
               Yoshua Bengio},
  editor    = {Francis R. Bach and
               David M. Blei},
  title     = {Show, Attend and Tell: Neural Image Caption Generation with Visual
               Attention},
  booktitle = {Proceedings of the 32nd International Conference on Machine Learning,
               {ICML} 2015, Lille, France, 6-11 July 2015},
  series    = {{JMLR} Workshop and Conference Proceedings},
  volume    = {37},
  pages     = {2048--2057},
  publisher = {JMLR.org},
  year      = {2015},
  url       = {http://proceedings.mlr.press/v37/xuc15.html},
  timestamp = {Wed, 29 May 2019 08:41:46 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/XuBKCCSZB15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{attention_bahdanau,
  author    = {Dzmitry Bahdanau and
               Kyunghyun Cho and
               Yoshua Bengio},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Neural Machine Translation by Jointly Learning to Align and Translate},
  booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
               San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
  year      = {2015},
  url       = {http://arxiv.org/abs/1409.0473},
  timestamp = {Wed, 17 Jul 2019 10:40:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/BahdanauCB14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{knowing_when_to_look,
  author    = {Jiasen Lu and
               Caiming Xiong and
               Devi Parikh and
               Richard Socher},
  title     = {Knowing When to Look: Adaptive Attention via a Visual Sentinel for
               Image Captioning},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {3242--3250},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.345},
  doi       = {10.1109/CVPR.2017.345},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/LuXPS17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{ask_attend_answer,
  author    = {Huijuan Xu and
               Kate Saenko},
  editor    = {Bastian Leibe and
               Jiri Matas and
               Nicu Sebe and
               Max Welling},
  title     = {Ask, Attend and Answer: Exploring Question-Guided Spatial Attention
               for Visual Question Answering},
  booktitle = {Computer Vision - {ECCV} 2016 - 14th European Conference, Amsterdam,
               The Netherlands, October 11-14, 2016, Proceedings, Part {VII}},
  series    = {Lecture Notes in Computer Science},
  volume    = {9911},
  pages     = {451--466},
  publisher = {Springer},
  year      = {2016},
  url       = {https://doi.org/10.1007/978-3-319-46478-7\_28},
  doi       = {10.1007/978-3-319-46478-7\_28},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/XuS16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{coattention_vqa,
  author    = {Jiasen Lu and
               Jianwei Yang and
               Dhruv Batra and
               Devi Parikh},
  editor    = {Daniel D. Lee and
               Masashi Sugiyama and
               Ulrike von Luxburg and
               Isabelle Guyon and
               Roman Garnett},
  title     = {Hierarchical Question-Image Co-Attention for Visual Question Answering},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {289--297},
  year      = {2016},
  url       = {http://papers.nips.cc/paper/6202-hierarchical-question-image-co-attention-for-visual-question-answering},
  timestamp = {Fri, 06 Mar 2020 17:00:15 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/LuYBP16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{stacked_attention_question_answering,
  author    = {Zichao Yang and
               Xiaodong He and
               Jianfeng Gao and
               Li Deng and
               Alexander J. Smola},
  title     = {Stacked Attention Networks for Image Question Answering},
  booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016},
  pages     = {21--29},
  publisher = {{IEEE} Computer Society},
  year      = {2016},
  url       = {https://doi.org/10.1109/CVPR.2016.10},
  doi       = {10.1109/CVPR.2016.10},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/YangHGDS16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{infoGAN,
  author    = {Xi Chen and
               Yan Duan and
               Rein Houthooft and
               John Schulman and
               Ilya Sutskever and
               Pieter Abbeel},
  editor    = {Daniel D. Lee and
               Masashi Sugiyama and
               Ulrike von Luxburg and
               Isabelle Guyon and
               Roman Garnett},
  title     = {InfoGAN: Interpretable Representation Learning by Information Maximizing
               Generative Adversarial Nets},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {2172--2180},
  year      = {2016},
  url       = {http://papers.nips.cc/paper/6399-infogan-interpretable-representation-learning-by-information-maximizing-generative-adversarial-nets},
  timestamp = {Fri, 06 Mar 2020 17:00:15 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/ChenCDHSSA16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{beta_vae,
  author    = {Irina Higgins and
               Lo{\"{\i}}c Matthey and
               Arka Pal and
               Christopher Burgess and
               Xavier Glorot and
               Matthew Botvinick and
               Shakir Mohamed and
               Alexander Lerchner},
  title     = {beta-VAE: Learning Basic Visual Concepts with a Constrained Variational
               Framework},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
               Toulon, France, April 24-26, 2017, Conference Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2017},
  url       = {https://openreview.net/forum?id=Sy2fzU9gl},
  timestamp = {Thu, 25 Jul 2019 14:25:41 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/HigginsMPBGBML17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{criticism_interpretability,
  author    = {Been Kim and
               Oluwasanmi Koyejo and
               Rajiv Khanna},
  editor    = {Daniel D. Lee and
               Masashi Sugiyama and
               Ulrike von Luxburg and
               Isabelle Guyon and
               Roman Garnett},
  title     = {Examples are not enough, learn to criticize! Criticism for Interpretability},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {2280--2288},
  year      = {2016},
  url       = {http://papers.nips.cc/paper/6300-examples-are-not-enough-learn-to-criticize-criticism-for-interpretability},
  timestamp = {Fri, 06 Mar 2020 17:00:15 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/KimKK16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{deep_inside_cnn,
  author    = {Karen Simonyan and
               Andrea Vedaldi and
               Andrew Zisserman},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Deep Inside Convolutional Networks: Visualising Image Classification
               Models and Saliency Maps},
  booktitle = {2nd International Conference on Learning Representations, {ICLR} 2014,
               Banff, AB, Canada, April 14-16, 2014, Workshop Track Proceedings},
  year      = {2014},
  url       = {http://arxiv.org/abs/1312.6034},
  timestamp = {Thu, 25 Jul 2019 14:36:46 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/SimonyanVZ13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{extracting_tree_structures,
  author    = {Mark W. Craven and
               Jude W. Shavlik},
  editor    = {David S. Touretzky and
               Michael Mozer and
               Michael E. Hasselmo},
  title     = {Extracting Tree-Structured Representations of Trained Networks},
  booktitle = {Advances in Neural Information Processing Systems 8, NIPS, Denver,
               CO, USA, November 27-30, 1995},
  pages     = {24--30},
  publisher = {{MIT} Press},
  year      = {1995},
  url       = {http://papers.nips.cc/paper/1152-extracting-tree-structured-representations-of-trained-networks},
  timestamp = {Fri, 06 Mar 2020 17:00:42 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/CravenS95.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{extracting_rules,
  author    = {Geoffrey G. Towell and
               Jude W. Shavlik},
  title     = {Extracting Refined Rules from Knowledge-Based Neural Networks},
  journal   = {Mach. Learn.},
  volume    = {13},
  pages     = {71--101},
  year      = {1993},
  url       = {https://doi.org/10.1007/BF00993103},
  doi       = {10.1007/BF00993103},
  timestamp = {Mon, 02 Mar 2020 16:29:49 +0100},
  biburl    = {https://dblp.org/rec/journals/ml/TowellS93.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{rule_based_ml,
  author    = {Sholom M. Weiss and
               Nitin Indurkhya},
  title     = {Rule-based Machine Learning Methods for Functional Prediction},
  journal   = {J. Artif. Intell. Res.},
  volume    = {3},
  pages     = {383--403},
  year      = {1995},
  url       = {https://doi.org/10.1613/jair.199},
  doi       = {10.1613/jair.199},
  timestamp = {Mon, 21 Jan 2019 15:01:17 +0100},
  biburl    = {https://dblp.org/rec/journals/jair/WeissI95.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@book{data_mining_decision_trees,
  author    = {Lior Rokach and
               Oded Maimon},
  title     = {Data Mining with Decision Trees - Theory and Applications. 2\({}^{\mbox{nd}}\)
               Edition},
  series    = {Series in Machine Perception and Artificial Intelligence},
  volume    = {81},
  publisher = {WorldScientific},
  year      = {2014},
  url       = {https://doi.org/10.1142/9097},
  doi       = {10.1142/9097},
  isbn      = {978-981-4590-07-5},
  timestamp = {Tue, 16 May 2017 14:24:22 +0200},
  biburl    = {https://dblp.org/rec/series/smpai/RokachM14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@incollection{linear_regression,
  author    = {Novi Quadrianto and
               Wray L. Buntine},
  editor    = {Claude Sammut and
               Geoffrey I. Webb},
  title     = {Linear Regression},
  booktitle = {Encyclopedia of Machine Learning},
  pages     = {603--606},
  publisher = {Springer},
  year      = {2010},
  url       = {https://doi.org/10.1007/978-0-387-30164-8\_476},
  doi       = {10.1007/978-0-387-30164-8\_476},
  timestamp = {Wed, 14 Nov 2018 10:51:34 +0100},
  biburl    = {https://dblp.org/rec/reference/ml/QuadriantoB10a.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{sanity_check_saliency,
  author    = {Julius Adebayo and
               Justin Gilmer and
               Michael Muelly and
               Ian J. Goodfellow and
               Moritz Hardt and
               Been Kim},
  editor    = {Samy Bengio and
               Hanna M. Wallach and
               Hugo Larochelle and
               Kristen Grauman and
               Nicol{\`{o}} Cesa{-}Bianchi and
               Roman Garnett},
  title     = {Sanity Checks for Saliency Maps},
  booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
               on Neural Information Processing Systems 2018, NeurIPS 2018, 3-8 December
               2018, Montr{\'{e}}al, Canada},
  pages     = {9525--9536},
  year      = {2018},
  url       = {http://papers.nips.cc/paper/8160-sanity-checks-for-saliency-maps},
  timestamp = {Fri, 06 Mar 2020 17:00:31 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/AdebayoGMGHK18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{interpretation_fragile,
  author    = {Amirata Ghorbani and
               Abubakar Abid and
               James Y. Zou},
  title     = {Interpretation of Neural Networks Is Fragile},
  booktitle = {The Thirty-Third {AAAI} Conference on Artificial Intelligence, {AAAI}
               2019, The Thirty-First Innovative Applications of Artificial Intelligence
               Conference, {IAAI} 2019, The Ninth {AAAI} Symposium on Educational
               Advances in Artificial Intelligence, {EAAI} 2019, Honolulu, Hawaii,
               USA, January 27 - February 1, 2019},
  pages     = {3681--3688},
  publisher = {{AAAI} Press},
  year      = {2019},
  url       = {https://doi.org/10.1609/aaai.v33i01.33013681},
  doi       = {10.1609/aaai.v33i01.33013681},
  timestamp = {Wed, 25 Sep 2019 11:05:08 +0200},
  biburl    = {https://dblp.org/rec/conf/aaai/GhorbaniAZ19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{attention_not_explanation,
  author    = {Sarthak Jain and
               Byron C. Wallace},
  editor    = {Jill Burstein and
               Christy Doran and
               Thamar Solorio},
  title     = {Attention is not Explanation},
  booktitle = {Proceedings of the 2019 Conference of the North American Chapter of
               the Association for Computational Linguistics: Human Language Technologies,
               {NAACL-HLT} 2019, Minneapolis, MN, USA, June 2-7, 2019, Volume 1 (Long
               and Short Papers)},
  pages     = {3543--3556},
  publisher = {Association for Computational Linguistics},
  year      = {2019},
  url       = {https://doi.org/10.18653/v1/n19-1357},
  doi       = {10.18653/v1/n19-1357},
  timestamp = {Tue, 28 Jan 2020 10:30:05 +0100},
  biburl    = {https://dblp.org/rec/conf/naacl/JainW19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{challenging_assumptions_disentangled,
  author    = {Francesco Locatello and
               Stefan Bauer and
               Mario Lucic and
               Gunnar R{\"{a}}tsch and
               Sylvain Gelly and
               Bernhard Sch{\"{o}}lkopf and
               Olivier Bachem},
  editor    = {Kamalika Chaudhuri and
               Ruslan Salakhutdinov},
  title     = {Challenging Common Assumptions in the Unsupervised Learning of Disentangled
               Representations},
  booktitle = {Proceedings of the 36th International Conference on Machine Learning,
               {ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
  series    = {Proceedings of Machine Learning Research},
  volume    = {97},
  pages     = {4114--4124},
  publisher = {{PMLR}},
  year      = {2019},
  url       = {http://proceedings.mlr.press/v97/locatello19a.html},
  timestamp = {Tue, 11 Jun 2019 15:37:38 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/LocatelloBLRGSB19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{soft_decision_tree,
  author    = {Nicholas Frosst and
               Geoffrey E. Hinton},
  editor    = {Tarek R. Besold and
               Oliver Kutz},
  title     = {Distilling a Neural Network Into a Soft Decision Tree},
  booktitle = {Proceedings of the First International Workshop on Comprehensibility
               and Explanation in {AI} and {ML} 2017 co-located with 16th International
               Conference of the Italian Association for Artificial Intelligence
               (AI*IA 2017), Bari, Italy, November 16th and 17th, 2017},
  series    = {{CEUR} Workshop Proceedings},
  volume    = {2071},
  publisher = {CEUR-WS.org},
  year      = {2017},
  url       = {http://ceur-ws.org/Vol-2071/CExAIIA\_2017\_paper\_3.pdf},
  timestamp = {Wed, 12 Feb 2020 16:44:29 +0100},
  biburl    = {https://dblp.org/rec/conf/aiia/FrosstH17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{interpreting_cnn_via_decision_trees,
  author    = {Quanshi Zhang and
               Yu Yang and
               Haotian Ma and
               Ying Nian Wu},
  title     = {Interpreting CNNs via Decision Trees},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {6261--6270},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Zhang\_Interpreting\_CNNs\_via\_Decision\_Trees\_CVPR\_2019\_paper.html},
  doi       = {10.1109/CVPR.2019.00642},
  timestamp = {Mon, 20 Jan 2020 15:36:04 +0100},
  biburl    = {https://dblp.org/rec/conf/cvpr/ZhangYMW19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{cnn_knowledge_explanatory_graph,
  author    = {Quanshi Zhang and
               Ruiming Cao and
               Feng Shi and
               Ying Nian Wu and
               Song{-}Chun Zhu},
  editor    = {Sheila A. McIlraith and
               Kilian Q. Weinberger},
  title     = {Interpreting {CNN} Knowledge via an Explanatory Graph},
  booktitle = {Proceedings of the Thirty-Second {AAAI} Conference on Artificial Intelligence,
               (AAAI-18), the 30th innovative Applications of Artificial Intelligence
               (IAAI-18), and the 8th {AAAI} Symposium on Educational Advances in
               Artificial Intelligence (EAAI-18), New Orleans, Louisiana, USA, February
               2-7, 2018},
  pages     = {4454--4463},
  publisher = {{AAAI} Press},
  year      = {2018},
  url       = {https://www.aaai.org/ocs/index.php/AAAI/AAAI18/paper/view/17354},
  timestamp = {Tue, 23 Oct 2018 06:42:15 +0200},
  biburl    = {https://dblp.org/rec/conf/aaai/ZhangCSWZ18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{recognition_to_cognition,
  author    = {Rowan Zellers and
               Yonatan Bisk and
               Ali Farhadi and
               Yejin Choi},
  title     = {From Recognition to Cognition: Visual Commonsense Reasoning},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {6720--6731},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Zellers\_From\_Recognition\_to\_Cognition\_Visual\_Commonsense\_Reasoning\_CVPR\_2019\_paper.html},
  doi       = {10.1109/CVPR.2019.00688},
  timestamp = {Mon, 20 Jan 2020 15:36:04 +0100},
  biburl    = {https://dblp.org/rec/conf/cvpr/ZellersBFC19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{explainable_nlp,
  author    = {Hui Liu and
               Qingyu Yin and
               William Yang Wang},
  editor    = {Anna Korhonen and
               David R. Traum and
               Llu{\'{\i}}s M{\`{a}}rquez},
  title     = {Towards Explainable {NLP:} {A} Generative Explanation Framework for
               Text Classification},
  booktitle = {Proceedings of the 57th Conference of the Association for Computational
               Linguistics, {ACL} 2019, Florence, Italy, July 28- August 2, 2019,
               Volume 1: Long Papers},
  pages     = {5570--5581},
  publisher = {Association for Computational Linguistics},
  year      = {2019},
  url       = {https://doi.org/10.18653/v1/p19-1560},
  doi       = {10.18653/v1/p19-1560},
  timestamp = {Tue, 28 Jan 2020 10:27:16 +0100},
  biburl    = {https://dblp.org/rec/conf/acl/LiuYW19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{esnli,
  author    = {Oana{-}Maria Camburu and
               Tim Rockt{\"{a}}schel and
               Thomas Lukasiewicz and
               Phil Blunsom},
  editor    = {Samy Bengio and
               Hanna M. Wallach and
               Hugo Larochelle and
               Kristen Grauman and
               Nicol{\`{o}} Cesa{-}Bianchi and
               Roman Garnett},
  title     = {e-SNLI: Natural Language Inference with Natural Language Explanations},
  booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
               on Neural Information Processing Systems 2018, NeurIPS 2018, 3-8 December
               2018, Montr{\'{e}}al, Canada},
  pages     = {9560--9572},
  year      = {2018},
  url       = {http://papers.nips.cc/paper/8163-e-snli-natural-language-inference-with-natural-language-explanations},
  timestamp = {Fri, 06 Mar 2020 17:00:31 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/CamburuRLB18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{nile,
  author    = {Sawan Kumar and
               Partha P. Talukdar},
  editor    = {Dan Jurafsky and
               Joyce Chai and
               Natalie Schluter and
               Joel R. Tetreault},
  title     = {{NILE} : Natural Language Inference with Faithful Natural Language
               Explanations},
  booktitle = {Proceedings of the 58th Annual Meeting of the Association for Computational
               Linguistics, {ACL} 2020, Online, July 5-10, 2020},
  pages     = {8730--8742},
  publisher = {Association for Computational Linguistics},
  year      = {2020},
  url       = {https://www.aclweb.org/anthology/2020.acl-main.771/},
  timestamp = {Wed, 24 Jun 2020 17:15:07 +0200},
  biburl    = {https://dblp.org/rec/conf/acl/KumarT20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{self_explaining_nn,
  author    = {David Alvarez{-}Melis and
               Tommi S. Jaakkola},
  editor    = {Samy Bengio and
               Hanna M. Wallach and
               Hugo Larochelle and
               Kristen Grauman and
               Nicol{\`{o}} Cesa{-}Bianchi and
               Roman Garnett},
  title     = {Towards Robust Interpretability with Self-Explaining Neural Networks},
  booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
               on Neural Information Processing Systems 2018, NeurIPS 2018, 3-8 December
               2018, Montr{\'{e}}al, Canada},
  pages     = {7786--7795},
  year      = {2018},
  url       = {http://papers.nips.cc/paper/8003-towards-robust-interpretability-with-self-explaining-neural-networks},
  timestamp = {Fri, 06 Mar 2020 17:00:31 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/Alvarez-MelisJ18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{explanation_object_detection,
  author    = {Thomas Ponn and
               Thomas Kr{\"{o}}ger and
               Frank Diermeyer},
  title     = {Identification and Explanation of Challenging Conditions for Camera-Based
               Object Detection of Automated Vehicles},
  journal   = {Sensors},
  volume    = {20},
  number    = {13},
  pages     = {3699},
  year      = {2020},
  url       = {https://doi.org/10.3390/s20133699},
  doi       = {10.3390/s20133699},
  timestamp = {Tue, 28 Jul 2020 14:03:49 +0200},
  biburl    = {https://dblp.org/rec/journals/sensors/PonnKD20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@book{molnar2019,
  title      = {Interpretable Machine Learning},
  author     = {Christoph Molnar},
  note       = {\url{https://christophm.github.io/interpretable-ml-book/}},
  year       = {2019},
  subtitle   = {A Guide for Making Black Box Models Explainable}
}

@inproceedings{partial_convolutions,
  author    = {Guilin Liu and
               Fitsum A. Reda and
               Kevin J. Shih and
               Ting{-}Chun Wang and
               Andrew Tao and
               Bryan Catanzaro},
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {Image Inpainting for Irregular Holes Using Partial Convolutions},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {XI}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11215},
  pages     = {89--105},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-01252-6\_6},
  doi       = {10.1007/978-3-030-01252-6\_6},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/LiuRSWTC18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{deeptest,
  author    = {Yuchi Tian and
               Kexin Pei and
               Suman Jana and
               Baishakhi Ray},
  editor    = {Michel Chaudron and
               Ivica Crnkovic and
               Marsha Chechik and
               Mark Harman},
  title     = {DeepTest: automated testing of deep-neural-network-driven autonomous
               cars},
  booktitle = {Proceedings of the 40th International Conference on Software Engineering,
               {ICSE} 2018, Gothenburg, Sweden, May 27 - June 03, 2018},
  pages     = {303--314},
  publisher = {{ACM}},
  year      = {2018},
  url       = {https://doi.org/10.1145/3180155.3180220},
  doi       = {10.1145/3180155.3180220},
  timestamp = {Wed, 16 Oct 2019 14:14:49 +0200},
  biburl    = {https://dblp.org/rec/conf/icse/TianPJR18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{safety_verification,
  author    = {Xiaowei Huang and
               Marta Kwiatkowska and
               Sen Wang and
               Min Wu},
  editor    = {Rupak Majumdar and
               Viktor Kuncak},
  title     = {Safety Verification of Deep Neural Networks},
  booktitle = {Computer Aided Verification - 29th International Conference, {CAV}
               2017, Heidelberg, Germany, July 24-28, 2017, Proceedings, Part {I}},
  series    = {Lecture Notes in Computer Science},
  volume    = {10426},
  pages     = {3--29},
  publisher = {Springer},
  year      = {2017},
  url       = {https://doi.org/10.1007/978-3-319-63387-9\_1},
  doi       = {10.1007/978-3-319-63387-9\_1},
  timestamp = {Wed, 04 Mar 2020 13:11:44 +0100},
  biburl    = {https://dblp.org/rec/conf/cav/HuangKWW17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{reluplex,
  author    = {Guy Katz and
               Clark W. Barrett and
               David L. Dill and
               Kyle Julian and
               Mykel J. Kochenderfer},
  editor    = {Rupak Majumdar and
               Viktor Kuncak},
  title     = {Reluplex: An Efficient {SMT} Solver for Verifying Deep Neural Networks},
  booktitle = {Computer Aided Verification - 29th International Conference, {CAV}
               2017, Heidelberg, Germany, July 24-28, 2017, Proceedings, Part {I}},
  series    = {Lecture Notes in Computer Science},
  volume    = {10426},
  pages     = {97--117},
  publisher = {Springer},
  year      = {2017},
  url       = {https://doi.org/10.1007/978-3-319-63387-9\_5},
  doi       = {10.1007/978-3-319-63387-9\_5},
  timestamp = {Wed, 25 Sep 2019 18:02:04 +0200},
  biburl    = {https://dblp.org/rec/conf/cav/KatzBDJK17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{deepxplore,
  author    = {Kexin Pei and
               Yinzhi Cao and
               Junfeng Yang and
               Suman Jana},
  title     = {DeepXplore: automated whitebox testing of deep learning systems},
  journal   = {Commun. {ACM}},
  volume    = {62},
  number    = {11},
  pages     = {137--145},
  year      = {2019},
  url       = {https://doi.org/10.1145/3361566},
  doi       = {10.1145/3361566},
  timestamp = {Tue, 05 Nov 2019 08:27:31 +0100},
  biburl    = {https://dblp.org/rec/journals/cacm/PeiCYJ19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{clustering_medoid,
  title={Clustering by means of medoids},
  author={Kaufmann, Leonard},
  booktitle={Proc. Statistical Data Analysis Based on the L1 Norm Conference, Neuchatel, 1987},
  pages={405--416},
  year={1987}
}

@article{tsne,
  title={Visualizing data using t-SNE},
  author={Maaten, Laurens van der and Hinton, Geoffrey},
  journal={Journal of machine learning research},
  volume={9},
  number={Nov},
  pages={2579--2605},
  year={2008}
}

@article{kitti,
  author    = {Andreas Geiger and
               Philip Lenz and
               Christoph Stiller and
               Raquel Urtasun},
  title     = {Vision meets robotics: The {KITTI} dataset},
  journal   = {I. J. Robotics Res.},
  volume    = {32},
  number    = {11},
  pages     = {1231--1237},
  year      = {2013},
  url       = {https://doi.org/10.1177/0278364913491297},
  doi       = {10.1177/0278364913491297},
  timestamp = {Thu, 18 May 2017 09:55:01 +0200},
  biburl    = {https://dblp.org/rec/journals/ijrr/GeigerLSU13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{CordtsORREBFRS16,
  author    = {Marius Cordts and
               Mohamed Omran and
               Sebastian Ramos and
               Timo Rehfeld and
               Markus Enzweiler and
               Rodrigo Benenson and
               Uwe Franke and
               Stefan Roth and
               Bernt Schiele},
  title     = {The Cityscapes Dataset for Semantic Urban Scene Understanding},
  journal   = {CoRR},
  volume    = {abs/1604.01685},
  year      = {2016},
  url       = {http://arxiv.org/abs/1604.01685},
  timestamp = {Wed, 07 Jun 2017 14:41:02 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/CordtsORREBFRS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}
@inproceedings{RosSMVL16,
  author    = {Germ{\'{a}}n Ros and
               Laura Sellart and
               Joanna Materzynska and
               David V{\'{a}}zquez and
               Antonio M. L{\'{o}}pez},
  title     = {The {SYNTHIA} Dataset: {A} Large Collection of Synthetic Images for
               Semantic Segmentation of Urban Scenes},
  booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016},
  pages     = {3234--3243},
  publisher = {{IEEE} Computer Society},
  year      = {2016},
  url       = {https://doi.org/10.1109/CVPR.2016.352},
  doi       = {10.1109/CVPR.2016.352},
  timestamp = {Tue, 05 Nov 2019 12:22:57 +0100},
  biburl    = {https://dblp.org/rec/conf/cvpr/RosSMVL16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{YuCWXCLMD20,
  author    = {Fisher Yu and
               Haofeng Chen and
               Xin Wang and
               Wenqi Xian and
               Yingying Chen and
               Fangchen Liu and
               Vashisht Madhavan and
               Trevor Darrell},
  title     = {{BDD100K:} {A} Diverse Driving Dataset for Heterogeneous Multitask
               Learning},
  booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
  pages     = {2633--2642},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/CVPR42600.2020.00271},
  doi       = {10.1109/CVPR42600.2020.00271},
  timestamp = {Tue, 11 Aug 2020 16:59:49 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/YuCWXCLMD20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{XiaZKNZW18,
  author    = {Ye Xia and
               Danqing Zhang and
               Jinkyu Kim and
               Ken Nakayama and
               Karl Zipser and
               David Whitney},
  editor    = {C. V. Jawahar and
               Hongdong Li and
               Greg Mori and
               Konrad Schindler},
  title     = {Predicting Driver Attention in Critical Situations},
  booktitle = {Computer Vision - {ACCV} 2018 - 14th Asian Conference on Computer
               Vision, Perth, Australia, December 2-6, 2018, Revised Selected Papers,
               Part {V}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11365},
  pages     = {658--674},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-20873-8\_42},
  doi       = {10.1007/978-3-030-20873-8\_42},
  timestamp = {Mon, 27 May 2019 13:56:09 +0200},
  biburl    = {https://dblp.org/rec/conf/accv/XiaZKNZW18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{RamanishkaCMS18,
  author    = {Vasili Ramanishka and
               Yi{-}Ting Chen and
               Teruhisa Misu and
               Kate Saenko},
  title     = {Toward Driving Scene Understanding: {A} Dataset for Learning Driver
               Behavior and Causal Reasoning},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {7699--7707},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Ramanishka\_Toward\_Driving\_Scene\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPR.2018.00803},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/RamanishkaCMS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{JainKSRSS16,
  author    = {Ashesh Jain and
               Hema Swetha Koppula and
               Shane Soh and
               Bharad Raghavan and
               Avi Singh and
               Ashutosh Saxena},
  title     = {Brain4Cars: Car That Knows Before You Do via Sensory-Fusion Deep Learning
               Architecture},
  journal   = {CoRR},
  volume    = {abs/1601.00740},
  year      = {2016},
  url       = {http://arxiv.org/abs/1601.00740},
  archivePrefix = {arXiv},
  eprint    = {1601.00740},
  timestamp = {Mon, 13 Aug 2018 16:46:15 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/JainKSRSS16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{CaesarBLVLXKPBB20,
  author    = {Holger Caesar and
               Varun Bankiti and
               Alex H. Lang and
               Sourabh Vora and
               Venice Erin Liong and
               Qiang Xu and
               Anush Krishnan and
               Yu Pan and
               Giancarlo Baldan and
               Oscar Beijbom},
  title     = {nuScenes: {A} Multimodal Dataset for Autonomous Driving},
  booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
  pages     = {11618--11628},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/CVPR42600.2020.01164},
  doi       = {10.1109/CVPR42600.2020.01164},
  timestamp = {Tue, 11 Aug 2020 16:59:49 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/CaesarBLVLXKPBB20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{HuangCGCZWLY18,
  author    = {Xinyu Huang and
               Xinjing Cheng and
               Qichuan Geng and
               Binbin Cao and
               Dingfu Zhou and
               Peng Wang and
               Yuanqing Lin and
               Ruigang Yang},
  title     = {The ApolloScape Dataset for Autonomous Driving},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition
               Workshops, {CVPR} Workshops 2018, Salt Lake City, UT, USA, June 18-22,
               2018},
  pages     = {954--960},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://openaccess.thecvf.com/content\_cvpr\_2018\_workshops/w14/html/Huang\_The\_ApolloScape\_Dataset\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPRW.2018.00141},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/HuangCGCZWLY18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{abs-2006-14480,
  author    = {John Houston and
               Guido Zuidhof and
               Luca Bergamini and
               Yawei Ye and
               Ashesh Jain and
               Sammy Omari and
               Vladimir Iglovikov and
               Peter Ondruska},
  title     = {One Thousand and One Hours: Self-driving Motion Prediction Dataset},
  journal   = {CoRR},
  volume    = {abs/2006.14480},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.14480},
  archivePrefix = {arXiv},
  eprint    = {2006.14480},
  timestamp = {Wed, 01 Jul 2020 15:21:23 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-14480.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{SunKDCPTGZCCVHN20,
  author    = {Pei Sun and
               Henrik Kretzschmar and
               Xerxes Dotiwalla and
               Aurelien Chouard and
               Vijaysai Patnaik and
               Paul Tsui and
               James Guo and
               Yin Zhou and
               Yuning Chai and
               Benjamin Caine and
               Vijay Vasudevan and
               Wei Han and
               Jiquan Ngiam and
               Hang Zhao and
               Aleksei Timofeev and
               Scott Ettinger and
               Maxim Krivokon and
               Amy Gao and
               Aditya Joshi and
               Yu Zhang and
               Jonathon Shlens and
               Zhifeng Chen and
               Dragomir Anguelov},
  title     = {Scalability in Perception for Autonomous Driving: Waymo Open Dataset},
  booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
  pages     = {2443--2451},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/CVPR42600.2020.00252},
  doi       = {10.1109/CVPR42600.2020.00252},
  timestamp = {Tue, 11 Aug 2020 16:59:49 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/SunKDCPTGZCCVHN20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{ChangLSSBHW0LRH19,
  author    = {Ming{-}Fang Chang and
               John Lambert and
               Patsorn Sangkloy and
               Jagjeet Singh and
               Slawomir Bak and
               Andrew Hartnett and
               De Wang and
               Peter Carr and
               Simon Lucey and
               Deva Ramanan and
               James Hays},
  title     = {Argoverse: 3D Tracking and Forecasting With Rich Maps},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {8748--8757},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Chang\_Argoverse\_3D\_Tracking\_and\_Forecasting\_With\_Rich\_Maps\_CVPR\_2019\_paper.html},
  doi       = {10.1109/CVPR.2019.00895},
  timestamp = {Mon, 20 Jan 2020 15:36:04 +0100},
  biburl    = {https://dblp.org/rec/conf/cvpr/ChangLSSBHW0LRH19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{abs-2004-03044,
  author    = {Yu Yao and
               Xizi Wang and
               Mingze Xu and
               Zelin Pu and
               Ella M. Atkins and
               David J. Crandall},
  title     = {When, Where, and What? {A} New Dataset for Anomaly Detection in Driving
               Videos},
  journal   = {CoRR},
  volume    = {abs/2004.03044},
  year      = {2020},
  url       = {https://arxiv.org/abs/2004.03044},
  archivePrefix = {arXiv},
  eprint    = {2004.03044},
  timestamp = {Wed, 08 Apr 2020 17:08:25 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2004-03044.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@techreport{LeCun04,
  added-at = {2008-03-11T14:52:34.000+0100},
  address = {http://www.cs.nyu.edu/\~{ }yann/research/dave/index.html},
  author = {Lecun, Y. and Cosatto, E. and Ben, J. and Muller, U. and Flepp, B.},
  biburl = {https://www.bibsonomy.org/bibtex/20e9a839118a9283db3986eb4723693a3/idsia},
  citeulike-article-id = {2380674},
  comment = {Presented at the Snowbird 2004 workshop},
  institution = {Courant Institute/CBLL},
  interhash = {28ab6c6a45d9fe306c7db64051c7c07b},
  intrahash = {0e9a839118a9283db3986eb4723693a3},
  keywords = {juergen},
  number = {DARPA-IPTO Final Report},
  priority = {2},
  timestamp = {2008-03-11T14:55:38.000+0100},
  title = {DAVE: Autonomous Off-Road Vehicle Control Using End-to-End Learning},
  year = 2004
}

@inproceedings{SrikanthARSMK19,
  author    = {Shashank Srikanth and
               Junaid Ahmed Ansari and
               Karnik Ram R. and
               Sarthak Sharma and
               J. Krishna Murthy and
               K. Madhava Krishna},
  title     = {{INFER:} INtermediate representations for FuturE pRediction},
  booktitle = {2019 {IEEE/RSJ} International Conference on Intelligent Robots and
               Systems, {IROS} 2019, Macau, SAR, China, November 3-8, 2019},
  pages     = {942--949},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/IROS40897.2019.8968553},
  doi       = {10.1109/IROS40897.2019.8968553},
  timestamp = {Thu, 30 Apr 2020 16:42:29 +0200},
  biburl    = {https://dblp.org/rec/conf/iros/SrikanthARSMK19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{RhinehartMKL19,
  author    = {Nicholas Rhinehart and
               Rowan McAllister and
               Kris Kitani and
               Sergey Levine},
  title     = {{PRECOG:} PREdiction Conditioned on Goals in Visual Multi-Agent Settings},
  booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
               2019, Seoul, Korea (South), October 27 - November 2, 2019},
  pages     = {2821--2830},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICCV.2019.00291},
  doi       = {10.1109/ICCV.2019.00291},
  timestamp = {Thu, 05 Mar 2020 13:43:22 +0100},
  biburl    = {https://dblp.org/rec/conf/iccv/RhinehartMKL19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{flatmobiles,
  author    = {Abdelhak Loukkal and
               Yves Grandvalet and
               Tom Drummond and
               You Li},
  title     = {Driving among Flatmobiles: Bird-Eye-View occupancy grids from a monocular
               camera for holistic trajectory planning},
  journal   = {CoRR},
  volume    = {abs/2008.04047},
  year      = {2020},
  url       = {https://arxiv.org/abs/2008.04047},
  archivePrefix = {arXiv},
  eprint    = {2008.04047},
  timestamp = {Fri, 14 Aug 2020 15:14:45 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2008-04047.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{trafficaccident,
  title={Traffic Accident Benchmark for Causality Recognition},
  author={You, Tackgeun and Han, Bohyung},
  year      = {2020},
}

@article{leeandsee2004,
author = {John D. Lee and Katrina A. See},
title ={Trust in Automation: Designing for Appropriate Reliance},
journal = {Human Factors},
volume = {46},
number = {1},
pages = {50-80},
year = {2004},
doi = {10.1518/hfes.46.1.50\_30392},
    note ={PMID: 15151155},
URL = {https://doi.org/10.1518/hfes.46.1.50_30392},
eprint = {https://doi.org/10.1518/hfes.46.1.50_30392}
}

@article{marshdibben20032,
author = {Marsh, Stephen and Dibben, Mark R.},
title = {The role of trust in information science and technology},
journal = {Annual Review of Information Science and Technology},
volume = {37},
number = {1},
pages = {465-498},
doi = {10.1002/aris.1440370111},
url = {https://asistdl.onlinelibrary.wiley.com/doi/abs/10.1002/aris.1440370111},
eprint = {https://asistdl.onlinelibrary.wiley.com/doi/pdf/10.1002/aris.1440370111},
year = {2003}
}

@article{action_based_representation,
  author    = {Yi Xiao and
               Felipe Codevilla and
               Christopher Pal and
               Antonio M. L{\'{o}}pez},
  title     = {Action-Based Representation Learning for Autonomous Driving},
  journal   = {CoRR},
  volume    = {abs/2008.09417},
  year      = {2020},
  url       = {https://arxiv.org/abs/2008.09417},
  archivePrefix = {arXiv},
  eprint    = {2008.09417},
  timestamp = {Fri, 28 Aug 2020 12:11:44 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2008-09417.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{perceive_predict_plan,
  author    = {Abbas Sadat and
               Sergio Casas and
               Mengye Ren and
               Xinyu Wu and
               Pranaab Dhawan and
               Raquel Urtasun},
  title     = {Perceive, Predict, and Plan: Safe Motion Planning Through Interpretable
               Semantic Representations},
  journal   = {CoRR},
  volume    = {abs/2008.05930},
  year      = {2020},
  url       = {https://arxiv.org/abs/2008.05930},
  archivePrefix = {arXiv},
  eprint    = {2008.05930},
  timestamp = {Mon, 17 Aug 2020 15:17:00 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2008-05930.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{deep_imitative_models,
  author    = {Nicholas Rhinehart and
               Rowan McAllister and
               Sergey Levine},
  title     = {Deep Imitative Models for Flexible Inference, Planning, and Control},
  booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
               Addis Ababa, Ethiopia, April 26-30, 2020},
  publisher = {OpenReview.net},
  year      = {2020},
  url       = {https://openreview.net/forum?id=Skl4mRNYDr},
  timestamp = {Thu, 07 May 2020 17:11:47 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/RhinehartML20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{xai_neuroscience,
  title={Explainable artificial intelligence for neuroscience: Behavioral neurostimulation},
  author={Fellous, Jean-Marc and Sapiro, Guillermo and Rossi, Andrew and Mayberg, Helen S and Ferrante, Michele},
  journal={Frontiers in Neuroscience},
  volume={13},
  pages={1346},
  year={2019},
  publisher={Frontiers}
}

@article{deeplearning_nature,
  author    = {Yann LeCun and
               Yoshua Bengio and
               Geoffrey E. Hinton},
  title     = {Deep learning},
  journal   = {Nat.},
  volume    = {521},
  number    = {7553},
  pages     = {436--444},
  year      = {2015},
  url       = {https://doi.org/10.1038/nature14539},
  doi       = {10.1038/nature14539},
  timestamp = {Mon, 08 Jun 2020 22:21:28 +0200},
  biburl    = {https://dblp.org/rec/journals/nature/LeCunBH15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{gan,
  author    = {Ian J. Goodfellow and
               Jean Pouget{-}Abadie and
               Mehdi Mirza and
               Bing Xu and
               David Warde{-}Farley and
               Sherjil Ozair and
               Aaron C. Courville and
               Yoshua Bengio},
  editor    = {Zoubin Ghahramani and
               Max Welling and
               Corinna Cortes and
               Neil D. Lawrence and
               Kilian Q. Weinberger},
  title     = {Generative Adversarial Nets},
  booktitle = {Advances in Neural Information Processing Systems 27: Annual Conference
               on Neural Information Processing Systems 2014, December 8-13 2014,
               Montreal, Quebec, Canada},
  pages     = {2672--2680},
  year      = {2014},
  url       = {http://papers.nips.cc/paper/5423-generative-adversarial-nets},
  timestamp = {Fri, 06 Mar 2020 16:58:17 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/GoodfellowPMXWOCB14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{survey_steering_angle,
  title={A Survey on Deep Learning for Steering Angle Prediction in Autonomous Vehicles},
  author={Manzo, Usman Gidado and Chiroma, Haruna and Aljojo, Nahla and Abubakar, Saidu and Popoola, Segun I and Al-Garadi, Mohammed Ali},
  journal={IEEE Access},
  year={2020},
  publisher={IEEE}
}

@article{mythos_interpretability,
  author    = {Zachary C. Lipton},
  title     = {The mythos of model interpretability},
  journal   = {Commun. {ACM}},
  volume    = {61},
  number    = {10},
  pages     = {36--43},
  year      = {2018},
  url       = {https://doi.org/10.1145/3233231},
  doi       = {10.1145/3233231},
  timestamp = {Wed, 21 Nov 2018 12:44:29 +0100},
  biburl    = {https://dblp.org/rec/journals/cacm/Lipton18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{intelligible_models_for_classification_and_regression,
  author    = {Yin Lou and
               Rich Caruana and
               Johannes Gehrke},
  editor    = {Qiang Yang and
               Deepak Agarwal and
               Jian Pei},
  title     = {Intelligible models for classification and regression},
  booktitle = {The 18th {ACM} {SIGKDD} International Conference on Knowledge Discovery
               and Data Mining, {KDD} '12, Beijing, China, August 12-16, 2012},
  pages     = {150--158},
  publisher = {{ACM}},
  year      = {2012},
  url       = {https://doi.org/10.1145/2339530.2339556},
  doi       = {10.1145/2339530.2339556},
  timestamp = {Tue, 06 Nov 2018 16:59:37 +0100},
  biburl    = {https://dblp.org/rec/conf/kdd/LouCG12.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{challenges_for_transparency,
  author    = {Adrian Weller},
  title     = {Challenges for Transparency},
  journal   = {CoRR},
  volume    = {abs/1708.01870},
  year      = {2017},
  url       = {http://arxiv.org/abs/1708.01870},
  archivePrefix = {arXiv},
  eprint    = {1708.01870},
  timestamp = {Mon, 13 Aug 2018 16:48:18 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1708-01870.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{towards_rigorous_science,
  title={Towards a rigorous science of interpretable machine learning},
  author={Doshi-Velez, Finale and Kim, Been},
  journal={arXiv preprint arXiv:1702.08608},
  year={2017}
}


@inproceedings{icarl,
  author    = {Sylvestre{-}Alvise Rebuffi and
               Alexander Kolesnikov and
               Georg Sperl and
               Christoph H. Lampert},
  title     = {iCaRL: Incremental Classifier and Representation Learning},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {5533--5542},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.587},
  doi       = {10.1109/CVPR.2017.587},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/RebuffiKSL17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{teaching_categories,
author = {Mac Aodha, Oisin and Su, Shihan and Chen, Yuxin and Perona, Pietro and Yue, Yisong},
title = {Teaching Categories to Human Learners With Visual Explanations},
booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2018}
}

@article{simson2017acm,
author = {Garfinkel, Simson and Matthews, Jeanna and Shapiro, Stuart S. and Smith, Jonathan M.},
title = {Toward Algorithmic Transparency and Accountability},
year = {2017},
issue_date = {September 2017},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {60},
number = {9},
issn = {0001-0782},
url = {https://doi.org/10.1145/3125780},
doi = {10.1145/3125780},
journal = {Commun. ACM},
month = aug,
pages = {5},
numpages = {1}
}

@inproceedings{rules_of_the_road,
  author    = {Joey Hong and
               Benjamin Sapp and
               James Philbin},
  title     = {Rules of the Road: Predicting Driving Behavior With a Convolutional
               Model of Semantic Interactions},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {8454--8462},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Hong\_Rules\_of\_the\_Road\_Predicting\_Driving\_Behavior\_With\_a\_Convolutional\_CVPR\_2019\_paper.html},
  doi       = {10.1109/CVPR.2019.00865},
  timestamp = {Thu, 27 Aug 2020 07:31:34 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/HongSP19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{borg2019safely,
  title={Safely Entering the Deep: A Review of Verification and Validation for Machine Learning and a Challenge Elicitation in the Automotive Industry},
  author={Borg, Markus and Englund, Cristofer and Wnuk, Krzysztof and Durann, Boris and Lewandowski, Christoffer and Gao, Shenjian and Tan, Yanwen and Kaijser, Henrik and L{\"o}nn, Henrik and T{\"o}rnqvist, Jonnas},
  journal={Journal of Automotive Software Engineering},
  volume={1},
  number={1},
  pages={1--19},
  year={2019},
  publisher={Atlantis Press}
}

@book{michon1984critical,
  title={A Critical View of Driver Behavior Models: What Do We Know, what Should We Do?},
  author={Michon, J.A.},
  url={https://books.google.fr/books?id=zWBzHAAACAAJ},
  year={1984}
}

@incollection{dataset_bias,
  author    = {Tatiana Tommasi and
               Novi Patricia and
               Barbara Caputo and
               Tinne Tuytelaars},
  editor    = {Gabriela Csurka},
  title     = {A Deeper Look at Dataset Bias},
  booktitle = {Domain Adaptation in Computer Vision Applications},
  series    = {Advances in Computer Vision and Pattern Recognition},
  pages     = {37--55},
  publisher = {Springer},
  year      = {2017},
  url       = {https://doi.org/10.1007/978-3-319-58347-1\_2},
  doi       = {10.1007/978-3-319-58347-1\_2},
  timestamp = {Fri, 02 Nov 2018 09:27:02 +0100},
  biburl    = {https://dblp.org/rec/series/acvpr/TommasiPCT17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{bias_fairness_ml,
  author    = {Ninareh Mehrabi and
               Fred Morstatter and
               Nripsuta Saxena and
               Kristina Lerman and
               Aram Galstyan},
  title     = {A Survey on Bias and Fairness in Machine Learning},
  journal   = {CoRR},
  volume    = {abs/1908.09635},
  year      = {2019},
  url       = {http://arxiv.org/abs/1908.09635},
  archivePrefix = {arXiv},
  eprint    = {1908.09635},
  timestamp = {Thu, 29 Aug 2019 16:32:34 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1908-09635.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{fooling_car_adversarial,
  author    = {Nir Morgulis and
               Alexander Kreines and
               Shachar Mendelowitz and
               Yuval Weisglass},
  title     = {Fooling a Real Car with Adversarial Traffic Signs},
  journal   = {CoRR},
  volume    = {abs/1907.00374},
  year      = {2019},
  url       = {http://arxiv.org/abs/1907.00374},
  archivePrefix = {arXiv},
  eprint    = {1907.00374},
  timestamp = {Mon, 08 Jul 2019 14:12:33 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1907-00374.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{adversarial_attacks_defenses_driving,
  author    = {Yao Deng and
               James Xi Zheng and
               Tianyi Zhang and
               Chen Chen and
               Guannan Lou and
               Miryung Kim},
  title     = {An Analysis of Adversarial Attacks and Defenses on Autonomous Driving
               Models},
  booktitle = {2020 {IEEE} International Conference on Pervasive Computing and Communications,
               PerCom 2020, Austin, TX, USA, March 23-27, 2020},
  pages     = {1--10},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/PerCom45495.2020.9127389},
  doi       = {10.1109/PerCom45495.2020.9127389},
  timestamp = {Thu, 16 Jul 2020 14:21:27 +0200},
  biburl    = {https://dblp.org/rec/conf/percom/DengZZCLK20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{anticipating_accidents_dashcam,
  author    = {Fu{-}Hsiang Chan and
               Yu{-}Ting Chen and
               Yu Xiang and
               Min Sun},
  editor    = {Shang{-}Hong Lai and
               Vincent Lepetit and
               Ko Nishino and
               Yoichi Sato},
  title     = {Anticipating Accidents in Dashcam Videos},
  booktitle = {Computer Vision - {ACCV} 2016 - 13th Asian Conference on Computer
               Vision, Taipei, Taiwan, November 20-24, 2016, Revised Selected Papers,
               Part {IV}},
  series    = {Lecture Notes in Computer Science},
  volume    = {10114},
  pages     = {136--153},
  publisher = {Springer},
  year      = {2016},
  url       = {https://doi.org/10.1007/978-3-319-54190-7\_9},
  doi       = {10.1007/978-3-319-54190-7\_9},
  timestamp = {Tue, 14 May 2019 10:00:50 +0200},
  biburl    = {https://dblp.org/rec/conf/accv/ChanCXS16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{agent_centric_risk_assessment,
  author    = {Kuo{-}Hao Zeng and
               Shih{-}Han Chou and
               Fu{-}Hsiang Chan and
               Juan Carlos Niebles and
               Min Sun},
  title     = {Agent-Centric Risk Assessment: Accident Anticipation and Risky Region
               Localization},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {1330--1338},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.146},
  doi       = {10.1109/CVPR.2017.146},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/ZengCCNS17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{SuzukiKAS18,
  author    = {Tomoyuki Suzuki and
               Hirokatsu Kataoka and
               Yoshimitsu Aoki and
               Yutaka Satoh},
  title     = {Anticipating Traffic Accidents With Adaptive Loss and Large-Scale
               Incident {DB}},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {3521--3529},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Suzuki\_Anticipating\_Traffic\_Accidents\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPR.2018.00371},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/SuzukiKAS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{KimLHS19,
  author    = {Hoon Kim and
               Kangwook Lee and
               Gyeongjo Hwang and
               Changho Suh},
  title     = {Crash to Not Crash: Learn to Identify Dangerous Vehicles Using a Simulator},
  booktitle = {The Thirty-Third {AAAI} Conference on Artificial Intelligence, {AAAI}
               2019, The Thirty-First Innovative Applications of Artificial Intelligence
               Conference, {IAAI} 2019, The Ninth {AAAI} Symposium on Educational
               Advances in Artificial Intelligence, {EAAI} 2019, Honolulu, Hawaii,
               USA, January 27 - February 1, 2019},
  pages     = {978--985},
  publisher = {{AAAI} Press},
  year      = {2019},
  url       = {https://doi.org/10.1609/aaai.v33i01.3301978},
  doi       = {10.1609/aaai.v33i01.3301978},
  timestamp = {Wed, 25 Sep 2019 11:05:08 +0200},
  biburl    = {https://dblp.org/rec/conf/aaai/KimLHS19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{representation_learning_review,
  author    = {Yoshua Bengio and
               Aaron C. Courville and
               Pascal Vincent},
  title     = {Representation Learning: {A} Review and New Perspectives},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {35},
  number    = {8},
  pages     = {1798--1828},
  year      = {2013},
  url       = {https://doi.org/10.1109/TPAMI.2013.50},
  doi       = {10.1109/TPAMI.2013.50},
  timestamp = {Wed, 14 Nov 2018 10:51:00 +0100},
  biburl    = {https://dblp.org/rec/journals/pami/BengioCV13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Espi2005TORCSTO,
  title={TORCS, The Open Racing Car Simulator},
  author={Eric Espi{\'e} and Christophe Guionneau and Bernhard Wymann and Christos Dimitrakakis and R{\'e}mi Coulom and A. Sumner},
  year={2005}
}

@article{drive_irl_dqn,
  author    = {Sahand Sharifzadeh and
               Ioannis Chiotellis and
               Rudolph Triebel and
               Daniel Cremers},
  title     = {Learning to Drive using Inverse Reinforcement Learning and Deep Q-Networks},
  journal   = {CoRR},
  volume    = {abs/1612.03653},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.03653},
  archivePrefix = {arXiv},
  eprint    = {1612.03653},
  timestamp = {Mon, 13 Aug 2018 16:48:50 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/SharifzadehCTC16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{algo_irl,
  author    = {Andrew Y. Ng and
               Stuart J. Russell},
  editor    = {Pat Langley},
  title     = {Algorithms for Inverse Reinforcement Learning},
  booktitle = {Proceedings of the Seventeenth International Conference on Machine
               Learning {(ICML} 2000), Stanford University, Stanford, CA, USA, June
               29 - July 2, 2000},
  pages     = {663--670},
  publisher = {Morgan Kaufmann},
  year      = {2000},
  timestamp = {Sun, 21 Feb 2010 20:54:50 +0100},
  biburl    = {https://dblp.org/rec/conf/icml/NgR00.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{deep_rl_driving_survey,
  author    = {Bangalore Ravi Kiran and
               Ibrahim Sobh and
               Victor Talpaert and
               Patrick Mannion and
               Ahmad A. Al Sallab and
               Senthil Kumar Yogamani and
               Patrick P{\'{e}}rez},
  title     = {Deep Reinforcement Learning for Autonomous Driving: {A} Survey},
  journal   = {CoRR},
  volume    = {abs/2002.00444},
  year      = {2020},
  url       = {https://arxiv.org/abs/2002.00444},
  archivePrefix = {arXiv},
  eprint    = {2002.00444},
  timestamp = {Mon, 10 Feb 2020 15:12:57 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2002-00444.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{gail,
  author    = {Jonathan Ho and
               Stefano Ermon},
  editor    = {Daniel D. Lee and
               Masashi Sugiyama and
               Ulrike von Luxburg and
               Isabelle Guyon and
               Roman Garnett},
  title     = {Generative Adversarial Imitation Learning},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {4565--4573},
  year      = {2016},
  url       = {http://papers.nips.cc/paper/6391-generative-adversarial-imitation-learning},
  timestamp = {Fri, 06 Mar 2020 17:00:15 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/HoE16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{driving_styles_demonstration,
  author    = {Markus Kuderer and
               Shilpa Gulati and
               Wolfram Burgard},
  title     = {Learning driving styles for autonomous vehicles from demonstration},
  booktitle = {{IEEE} International Conference on Robotics and Automation, {ICRA}
               2015, Seattle, WA, USA, 26-30 May, 2015},
  pages     = {2641--2646},
  publisher = {{IEEE}},
  year      = {2015},
  url       = {https://doi.org/10.1109/ICRA.2015.7139555},
  doi       = {10.1109/ICRA.2015.7139555},
  timestamp = {Sat, 05 Sep 2020 18:04:17 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/KudererGB15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{multimodal_experts_network,
  author    = {Shihong Fang and
               Anna Choromanska},
  title     = {Multi-modal Experts Network for Autonomous Driving},
  booktitle = {2020 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2020, Paris, France, May 31 - August 31, 2020},
  pages     = {6439--6445},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/ICRA40945.2020.9197459},
  doi       = {10.1109/ICRA40945.2020.9197459},
  timestamp = {Mon, 28 Sep 2020 12:19:28 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/FangC20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{effect_visualization_pedestrian_intention,
author = {Colley, Mark and Br\"{a}uner, Christian and Lanzer, Mirjam and Walch, Marcel and Baumann, Martin and Rukzio, Enrico},
title = {Effect of Visualization of Pedestrian Intention Recognition on Trust and Cognitive Load},
year = {2020},
isbn = {9781450380652},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3409120.3410648},
doi = {10.1145/3409120.3410648},
booktitle = {12th International Conference on Automotive User Interfaces and Interactive Vehicular Applications},
pages = {181–191},
numpages = {11},
keywords = {interface design., pedestrian intention, Autonomous vehicles},
location = {Virtual Event, DC, USA},
series = {AutomotiveUI '20}
}

@inproceedings{apprenticeship_irl,
  author    = {Pieter Abbeel and
               Andrew Y. Ng},
  editor    = {Carla E. Brodley},
  title     = {Apprenticeship learning via inverse reinforcement learning},
  booktitle = {Machine Learning, Proceedings of the Twenty-first International Conference
               {(ICML} 2004), Banff, Alberta, Canada, July 4-8, 2004},
  series    = {{ACM} International Conference Proceeding Series},
  volume    = {69},
  publisher = {{ACM}},
  year      = {2004},
  url       = {https://doi.org/10.1145/1015330.1015430},
  doi       = {10.1145/1015330.1015430},
  timestamp = {Tue, 06 Nov 2018 16:58:29 +0100},
  biburl    = {https://dblp.org/rec/conf/icml/PieterN04.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{game_theoretic_apprenticeship_learning,
  author    = {Umar Syed and
               Robert E. Schapire},
  editor    = {John C. Platt and
               Daphne Koller and
               Yoram Singer and
               Sam T. Roweis},
  title     = {A Game-Theoretic Approach to Apprenticeship Learning},
  booktitle = {Advances in Neural Information Processing Systems 20, Proceedings
               of the Twenty-First Annual Conference on Neural Information Processing
               Systems, Vancouver, British Columbia, Canada, December 3-6, 2007},
  pages     = {1449--1456},
  publisher = {Curran Associates, Inc.},
  year      = {2007},
  url       = {http://papers.nips.cc/paper/3293-a-game-theoretic-approach-to-apprenticeship-learning},
  timestamp = {Fri, 06 Mar 2020 16:59:32 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/SyedS07.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{apprenticeship_learning_motion_planning,
  author    = {Pieter Abbeel and
               Dmitri Dolgov and
               Andrew Y. Ng and
               Sebastian Thrun},
  title     = {Apprenticeship learning for motion planning with application to parking
               lot navigation},
  booktitle = {2008 {IEEE/RSJ} International Conference on Intelligent Robots and
               Systems, September 22-26, 2008, Acropolis Convention Center, Nice,
               France},
  pages     = {1083--1090},
  publisher = {{IEEE}},
  year      = {2008},
  url       = {https://doi.org/10.1109/IROS.2008.4651222},
  doi       = {10.1109/IROS.2008.4651222},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iros/AbbeelDNT08.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{maximum_entropy_irl,
  author    = {Brian D. Ziebart and
               Andrew L. Maas and
               J. Andrew Bagnell and
               Anind K. Dey},
  editor    = {Dieter Fox and
               Carla P. Gomes},
  title     = {Maximum Entropy Inverse Reinforcement Learning},
  booktitle = {Proceedings of the Twenty-Third {AAAI} Conference on Artificial Intelligence,
               {AAAI} 2008, Chicago, Illinois, USA, July 13-17, 2008},
  pages     = {1433--1438},
  publisher = {{AAAI} Press},
  year      = {2008},
  url       = {http://www.aaai.org/Library/AAAI/2008/aaai08-227.php},
  timestamp = {Mon, 10 Dec 2012 17:36:53 +0100},
  biburl    = {https://dblp.org/rec/conf/aaai/ZiebartMBD08.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@book{Gibson1979,
	author = {James J. Gibson},
	title = {The Ecological Approach to Visual Perception},
	publisher = {Houghton Mifflin},
	year = {1979}
}

@inproceedings{spatio_temporal_action_graph_networks,
  author    = {Roei Herzig and
               Elad Levi and
               Huijuan Xu and
               Hang Gao and
               Eli Brosh and
               Xiaolong Wang and
               Amir Globerson and
               Trevor Darrell},
  title     = {Spatio-Temporal Action Graph Networks},
  booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision Workshops,
               {ICCV} Workshops 2019, Seoul, Korea (South), October 27-28, 2019},
  pages     = {2347--2356},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICCVW.2019.00288},
  doi       = {10.1109/ICCVW.2019.00288},
  timestamp = {Thu, 12 Mar 2020 12:34:59 +0100},
  biburl    = {https://dblp.org/rec/conf/iccvw/HerzigLXGBWGD19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{drive_video_analysis_detection_of_traffic_near_miss_incidents,
  author    = {Hirokatsu Kataoka and
               Teppei Suzuki and
               Shoko Oikawa and
               Yasuhiro Matsui and
               Yutaka Satoh},
  title     = {Drive Video Analysis for the Detection of Traffic Near-Miss Incidents},
  booktitle = {2018 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2018, Brisbane, Australia, May 21-25, 2018},
  pages     = {1--8},
  publisher = {{IEEE}},
  year      = {2018},
  url       = {https://doi.org/10.1109/ICRA.2018.8460812},
  doi       = {10.1109/ICRA.2018.8460812},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/KataokaSOMS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{unsupervised_traffic_accident_detection,
  author    = {Yu Yao and
               Mingze Xu and
               Yuchen Wang and
               David J. Crandall and
               Ella M. Atkins},
  title     = {Unsupervised Traffic Accident Detection in First-Person Videos},
  booktitle = {2019 {IEEE/RSJ} International Conference on Intelligent Robots and
               Systems, {IROS} 2019, Macau, SAR, China, November 3-8, 2019},
  pages     = {273--280},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/IROS40897.2019.8967556},
  doi       = {10.1109/IROS40897.2019.8967556},
  timestamp = {Fri, 31 Jan 2020 13:28:16 +0100},
  biburl    = {https://dblp.org/rec/conf/iros/YaoXWCA19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{viena,
  author    = {Mohammad Sadegh Aliakbarian and
               Fatemeh Sadat Saleh and
               Mathieu Salzmann and
               Basura Fernando and
               Lars Petersson and
               Lars Andersson},
  editor    = {C. V. Jawahar and
               Hongdong Li and
               Greg Mori and
               Konrad Schindler},
  title     = {{VIENA} {\^{}}2 : {A} Driving Anticipation Dataset},
  booktitle = {Computer Vision - {ACCV} 2018 - 14th Asian Conference on Computer
               Vision, Perth, Australia, December 2-6, 2018, Revised Selected Papers,
               Part {I}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11361},
  pages     = {449--466},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-20887-5\_28},
  doi       = {10.1007/978-3-030-20887-5\_28},
  timestamp = {Tue, 28 May 2019 13:43:37 +0200},
  biburl    = {https://dblp.org/rec/conf/accv/AliakbarianSSFP18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{exploring_reactions_unexpected,
  title={“I’d like an Explanation for That!” Exploring Reactions to Unexpected Autonomous Driving},
  author={Wiegand, Gesa and Eiband, Malin and Haubelt, Maximilian and Hussmann, Heinrich},
  booktitle={22nd International Conference on Human-Computer Interaction with Mobile Devices and Services},
  pages={1--11},
  year={2020}
}

@article{leakage_adjusted_simulatability,
  title={Leakage-Adjusted Simulatability: Can Models Generate Non-Trivial Explanations of Their Behavior in Natural Language?},
  author={Hase, Peter and Zhang, Shiyue and Xie, Harry and Bansal, Mohit},
  journal={arXiv preprint arXiv:2010.04119},
  year={2020}
}

@article{aligning_faithful_interpretations,
  author    = {Alon Jacovi and
               Yoav Goldberg},
  title     = {Aligning Faithful Interpretations with their Social Attribution},
  journal   = {CoRR},
  volume    = {abs/2006.01067},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.01067},
  archivePrefix = {arXiv},
  eprint    = {2006.01067},
  timestamp = {Mon, 08 Jun 2020 15:48:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-01067.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{development_machine_vision,
  author={E. D. {Dickmanns}},
  booktitle={Intelligent Vehicle Symposium, 2002. IEEE}, 
  title={The development of machine vision for road vehicles in the last decade}, 
  year={2002},
  volume={1},
  number={},
  pages={268-281 vol.1},
  }
  
@article{perception_driven_autonomous,
  title={A perception-driven autonomous urban vehicle},
  author={Leonard, John and How, Jonathan and Teller, Seth and Berger, Mitch and Campbell, Stefan and Fiore, Gaston and Fletcher, Luke and Frazzoli, Emilio and Huang, Albert and Karaman, Sertac and others},
  journal={Journal of Field Robotics},
  volume={25},
  number={10},
  pages={727--774},
  year={2008},
  publisher={Wiley Online Library}
}

@inproceedings{imagenet_classification,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle={Advances in neural information processing systems},
  pages={1097--1105},
  year={2012}
}

@inproceedings{adversarial_examples_are_not_bugs,
  title={Adversarial examples are not bugs, they are features},
  author={Ilyas, Andrew and Santurkar, Shibani and Tsipras, Dimitris and Engstrom, Logan and Tran, Brandon and Madry, Aleksander},
  booktitle={Advances in Neural Information Processing Systems},
  pages={125--136},
  year={2019}
}

@inproceedings{interpretable_neural_predictions,
  author    = {Jasmijn Bastings and
               Wilker Aziz and
               Ivan Titov},
  editor    = {Anna Korhonen and
               David R. Traum and
               Llu{\'{\i}}s M{\`{a}}rquez},
  title     = {Interpretable Neural Predictions with Differentiable Binary Variables},
  booktitle = {Proceedings of the 57th Conference of the Association for Computational
               Linguistics, {ACL} 2019, Florence, Italy, July 28- August 2, 2019,
               Volume 1: Long Papers},
  pages     = {2963--2977},
  publisher = {Association for Computational Linguistics},
  year      = {2019},
  url       = {https://doi.org/10.18653/v1/p19-1284},
  doi       = {10.18653/v1/p19-1284},
  timestamp = {Tue, 14 Jul 2020 12:30:14 +0200},
  biburl    = {https://dblp.org/rec/conf/acl/BastingsAT19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{learning_to_faithfully_rationalize,
  author    = {Sarthak Jain and
               Sarah Wiegreffe and
               Yuval Pinter and
               Byron C. Wallace},
  editor    = {Dan Jurafsky and
               Joyce Chai and
               Natalie Schluter and
               Joel R. Tetreault},
  title     = {Learning to Faithfully Rationalize by Construction},
  booktitle = {Proceedings of the 58th Annual Meeting of the Association for Computational
               Linguistics, {ACL} 2020, Online, July 5-10, 2020},
  pages     = {4459--4473},
  publisher = {Association for Computational Linguistics},
  year      = {2020},
  url       = {https://www.aclweb.org/anthology/2020.acl-main.409/},
  timestamp = {Wed, 24 Jun 2020 17:15:07 +0200},
  biburl    = {https://dblp.org/rec/conf/acl/JainWPW20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{please_stop_explaining_black_box_models,
  author    = {Cynthia Rudin},
  title     = {Please Stop Explaining Black Box Models for High Stakes Decisions},
  journal   = {CoRR},
  volume    = {abs/1811.10154},
  year      = {2018},
  url       = {http://arxiv.org/abs/1811.10154},
  archivePrefix = {arXiv},
  eprint    = {1811.10154},
  timestamp = {Fri, 30 Nov 2018 14:31:38 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1811-10154.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{explanation_in_ai,
  author    = {Tim Miller},
  title     = {Explanation in artificial intelligence: Insights from the social sciences},
  journal   = {Artif. Intell.},
  volume    = {267},
  pages     = {1--38},
  year      = {2019},
  url       = {https://doi.org/10.1016/j.artint.2018.07.007},
  doi       = {10.1016/j.artint.2018.07.007},
  timestamp = {Wed, 09 Jan 2019 15:42:37 +0100},
  biburl    = {https://dblp.org/rec/journals/ai/Miller19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{promise_and_peril_human_eval,
  author    = {Bernease Herman},
  title     = {The Promise and Peril of Human Evaluation for Model Interpretability},
  journal   = {CoRR},
  volume    = {abs/1711.07414},
  year      = {2017},
  url       = {http://arxiv.org/abs/1711.07414},
  archivePrefix = {arXiv},
  eprint    = {1711.07414},
  timestamp = {Tue, 05 Nov 2019 14:27:19 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1711-07414.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{darts_deceiving_autonomous,
  author    = {Chawin Sitawarin and
               Arjun Nitin Bhagoji and
               Arsalan Mosenia and
               Mung Chiang and
               Prateek Mittal},
  title     = {{DARTS:} Deceiving Autonomous Cars with Toxic Signs},
  journal   = {CoRR},
  volume    = {abs/1802.06430},
  year      = {2018},
  url       = {http://arxiv.org/abs/1802.06430},
  archivePrefix = {arXiv},
  eprint    = {1802.06430},
  timestamp = {Mon, 13 Aug 2018 16:48:27 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1802-06430.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{analysis_adversarial_attacks,
  author    = {Yao Deng and
               James Xi Zheng and
               Tianyi Zhang and
               Chen Chen and
               Guannan Lou and
               Miryung Kim},
  title     = {An Analysis of Adversarial Attacks and Defenses on Autonomous Driving
               Models},
  booktitle = {2020 {IEEE} International Conference on Pervasive Computing and Communications,
               PerCom 2020, Austin, TX, USA, March 23-27, 2020},
  pages     = {1--10},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/PerCom45495.2020.9127389},
  doi       = {10.1109/PerCom45495.2020.9127389},
  timestamp = {Thu, 16 Jul 2020 14:21:27 +0200},
  biburl    = {https://dblp.org/rec/conf/percom/DengZZCLK20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{states_versus_rewards,
  title={States versus rewards: dissociable neural prediction error signals underlying model-based and model-free reinforcement learning},
  author={Gl{\"a}scher, Jan and Daw, Nathaniel and Dayan, Peter and O'Doherty, John P},
  journal={Neuron},
  volume={66},
  number={4},
  pages={585--595},
  year={2010},
  publisher={Elsevier}
}

@article{separate_encoding_model_based,
  title={Separate encoding of model-based and model-free valuations in the human brain},
  author={Beierholm, Ulrik R and Anen, Cedric and Quartz, Steven and Bossaerts, Peter},
  journal={Neuroimage},
  volume={58},
  number={3},
  pages={955--962},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{bleu,
  author    = {Kishore Papineni and
               Salim Roukos and
               Todd Ward and
               Wei{-}Jing Zhu},
  title     = {Bleu: a Method for Automatic Evaluation of Machine Translation},
  booktitle = {Proceedings of the 40th Annual Meeting of the Association for Computational
               Linguistics, July 6-12, 2002, Philadelphia, PA, {USA}},
  pages     = {311--318},
  year      = {2002},
  crossref  = {DBLP:conf/acl/2002},
  url       = {https://www.aclweb.org/anthology/P02-1040/},
  timestamp = {Tue, 17 Sep 2019 13:40:53 +0200},
  biburl    = {https://dblp.org/rec/conf/acl/PapineniRWZ02.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{meteor,
  author    = {Satanjeev Banerjee and
               Alon Lavie},
  title     = {{METEOR:} An Automatic Metric for {MT} Evaluation with Improved Correlation
               with Human Judgments},
  booktitle = {Proceedings of the Workshop on Intrinsic and Extrinsic Evaluation
               Measures for Machine Translation and/or Summarization@ACL 2005, Ann
               Arbor, Michigan, USA, June 29, 2005},
  pages     = {65--72},
  year      = {2005},
  crossref  = {DBLP:conf/acl/2005ee},
  url       = {https://www.aclweb.org/anthology/W05-0909/},
  timestamp = {Wed, 11 Sep 2019 16:27:20 +0200},
  biburl    = {https://dblp.org/rec/conf/acl/BanerjeeL05.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{explain_yourself,
  author    = {Nazneen Fatema Rajani and
               Bryan McCann and
               Caiming Xiong and
               Richard Socher},
  editor    = {Anna Korhonen and
               David R. Traum and
               Llu{\'{\i}}s M{\`{a}}rquez},
  title     = {Explain Yourself! Leveraging Language Models for Commonsense Reasoning},
  booktitle = {Proceedings of the 57th Conference of the Association for Computational
               Linguistics, {ACL} 2019, Florence, Italy, July 28- August 2, 2019,
               Volume 1: Long Papers},
  pages     = {4932--4942},
  publisher = {Association for Computational Linguistics},
  year      = {2019},
  url       = {https://doi.org/10.18653/v1/p19-1487},
  doi       = {10.18653/v1/p19-1487},
  timestamp = {Tue, 28 Jan 2020 10:27:59 +0100},
  biburl    = {https://dblp.org/rec/conf/acl/RajaniMXS19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{real_to_virtual_domain_unification,
  author    = {Luona Yang and
               Xiaodan Liang and
               Tairui Wang and
               Eric P. Xing},
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {Real-to-Virtual Domain Unification for End-to-End Autonomous Driving},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {IV}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11208},
  pages     = {553--570},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-01225-0\_33},
  doi       = {10.1007/978-3-030-01225-0\_33},
  timestamp = {Mon, 22 Jul 2019 16:49:12 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/YangLWX18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{training_my_car_to_see,
  author    = {Antonio M. L{\'{o}}pez and
               Gabriel Villalonga and
               Laura Sellart and
               Germ{\'{a}}n Ros and
               David V{\'{a}}zquez and
               Jiaolong Xu and
               Javier Mar{\'{\i}}n and
               Azadeh Sadat Mozafari},
  title     = {Training my car to see using virtual worlds},
  journal   = {Image Vis. Comput.},
  volume    = {68},
  pages     = {102--118},
  year      = {2017},
  url       = {https://doi.org/10.1016/j.imavis.2017.07.007},
  doi       = {10.1016/j.imavis.2017.07.007},
  timestamp = {Thu, 20 Feb 2020 09:11:09 +0100},
  biburl    = {https://dblp.org/rec/journals/ivc/LopezVSRVXMM17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{no_regret_reductions,
  author    = {St{\'{e}}phane Ross and
               Geoffrey J. Gordon and
               J. Andrew Bagnell},
  title     = {No-Regret Reductions for Imitation Learning and Structured Prediction},
  journal   = {CoRR},
  volume    = {abs/1011.0686},
  year      = {2010},
  url       = {http://arxiv.org/abs/1011.0686},
  archivePrefix = {arXiv},
  eprint    = {1011.0686},
  timestamp = {Mon, 13 Aug 2018 16:45:56 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1011-0686.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{discovering_causal_signals_images,
  author    = {David Lopez{-}Paz and
               Robert Nishihara and
               Soumith Chintala and
               Bernhard Sch{\"{o}}lkopf and
               L{\'{e}}on Bottou},
  title     = {Discovering Causal Signals in Images},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {58--66},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.14},
  doi       = {10.1109/CVPR.2017.14},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/Lopez-PazNCSB17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{learning_representations_using_causal_invariance,
  author    = {L{\'{e}}on Bottou},
  editor    = {Antoine Cornu{\'{e}}jols and
               Etienne Cuvelier},
  title     = {Learning Representations Using Causal Invariance},
  booktitle = {Extraction et Gestion des Connaissances, {EGC} 2020, Brussels, Belgium,
               January 27-31, 2020},
  series    = {{RNTI}},
  volume    = {{E-36}},
  pages     = {5--6},
  publisher = {{\'{E}}ditions {RNTI}},
  year      = {2020},
  url       = {http://editions-rnti.fr/?inprocid=1002554},
  timestamp = {Tue, 09 Jun 2020 18:37:43 +0200},
  biburl    = {https://dblp.org/rec/conf/f-egc/Bottou20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{study_multimodal_interactive_vqa,
  author    = {Kamran Alipour and
               J{\"{u}}rgen P. Schulze and
               Yi Yao and
               Avi Ziskind and
               Giedrius Burachas},
  editor    = {Hu{\'{a}}scar Espinoza and
               Jos{\'{e}} Hern{\'{a}}ndez{-}Orallo and
               Xin Cynthia Chen and
               Se{\'{a}}n S. {\'{O}}h{\'{E}}igeartaigh and
               Xiaowei Huang and
               Mauricio Castillo{-}Effen and
               Richard Mallah and
               John McDermid},
  title     = {A Study on Multimodal and Interactive Explanations for Visual Question
               Answering},
  booktitle = {Proceedings of the Workshop on Artificial Intelligence Safety, co-located
               with 34th {AAAI} Conference on Artificial Intelligence, SafeAI@AAAI
               2020, New York City, NY, USA, February 7, 2020},
  series    = {{CEUR} Workshop Proceedings},
  volume    = {2560},
  pages     = {54--62},
  publisher = {CEUR-WS.org},
  year      = {2020},
  url       = {http://ceur-ws.org/Vol-2560/paper44.pdf},
  timestamp = {Fri, 06 Mar 2020 12:47:03 +0100},
  biburl    = {https://dblp.org/rec/conf/aaai/AlipourSYZB20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{manigan,
  author    = {Bowen Li and
               Xiaojuan Qi and
               Thomas Lukasiewicz and
               Philip H. S. Torr},
  title     = {ManiGAN: Text-Guided Image Manipulation},
  booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
  pages     = {7877--7886},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/CVPR42600.2020.00790},
  doi       = {10.1109/CVPR42600.2020.00790},
  timestamp = {Tue, 11 Aug 2020 16:59:49 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/LiQLT20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{lightweight_gan_text_guided,
  title={Lightweight Generative Adversarial Networks for Text- Guided Image Manipulation},
  author={Li, Bowen and Lukasiewicz, Thomas},
  year={2020}
}

@incollection{cord,
  author    = {Matthieu Cord and
               Philippe Henri Gosselin},
  editor    = {Matthieu Cord and
               P{\'{a}}draig Cunningham},
  title     = {Online Content-Based Image Retrieval Using Active Learning},
  booktitle = {Machine Learning Techniques for Multimedia - Case Studies on Organization
               and Retrieval},
  series    = {Cognitive Technologies},
  pages     = {115--138},
  publisher = {Springer},
  year      = {2008},
  url       = {https://doi.org/10.1007/978-3-540-75171-7\_5},
  doi       = {10.1007/978-3-540-75171-7\_5},
  timestamp = {Wed, 14 Jun 2017 20:39:09 +0200},
  biburl    = {https://dblp.org/rec/series/cogtech/CordG08.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{cnn_features_off_the_shelf,
  author    = {Ali Sharif Razavian and
               Hossein Azizpour and
               Josephine Sullivan and
               Stefan Carlsson},
  title     = {{CNN} Features Off-the-Shelf: An Astounding Baseline for Recognition},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               Workshops 2014, Columbus, OH, USA, June 23-28, 2014},
  pages     = {512--519},
  publisher = {{IEEE} Computer Society},
  year      = {2014},
  url       = {https://doi.org/10.1109/CVPRW.2014.131},
  doi       = {10.1109/CVPRW.2014.131},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/RazavianASC14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{C3D,
  author    = {Du Tran and
               Lubomir D. Bourdev and
               Rob Fergus and
               Lorenzo Torresani and
               Manohar Paluri},
  title     = {Learning Spatiotemporal Features with 3D Convolutional Networks},
  booktitle = {2015 {IEEE} International Conference on Computer Vision, {ICCV} 2015,
               Santiago, Chile, December 7-13, 2015},
  pages     = {4489--4497},
  publisher = {{IEEE} Computer Society},
  year      = {2015},
  url       = {https://doi.org/10.1109/ICCV.2015.510},
  doi       = {10.1109/ICCV.2015.510},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iccv/TranBFTP15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{graying_black_box,
  author    = {Tom Zahavy and
               Nir Ben{-}Zrihem and
               Shie Mannor},
  editor    = {Maria{-}Florina Balcan and
               Kilian Q. Weinberger},
  title     = {Graying the black box: Understanding DQNs},
  booktitle = {Proceedings of the 33nd International Conference on Machine Learning,
               {ICML} 2016, New York City, NY, USA, June 19-24, 2016},
  series    = {{JMLR} Workshop and Conference Proceedings},
  volume    = {48},
  pages     = {1899--1908},
  publisher = {JMLR.org},
  year      = {2016},
  url       = {http://proceedings.mlr.press/v48/zahavy16.html},
  timestamp = {Wed, 29 May 2019 08:41:46 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/ZahavyBM16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{visual_interpretability_dl_survey,
  author    = {Quanshi Zhang and
               Song{-}Chun Zhu},
  title     = {Visual interpretability for deep learning: a survey},
  journal   = {Frontiers Inf. Technol. Electron. Eng.},
  volume    = {19},
  number    = {1},
  pages     = {27--39},
  year      = {2018},
  url       = {https://doi.org/10.1631/FITEE.1700808},
  doi       = {10.1631/FITEE.1700808},
  timestamp = {Thu, 05 Mar 2020 17:10:30 +0100},
  biburl    = {https://dblp.org/rec/journals/jzusc/ZhangZ18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{visualizing_higher_layer_features,
  title={Visualizing higher-layer features of a deep network},
  author={Erhan, Dumitru and Bengio, Yoshua and Courville, Aaron and Vincent, Pascal},
  journal={University of Montreal},
  volume={1341},
  number={3},
  pages={1},
  year={2009}
}

@inproceedings{synthesizing_preferred_inputs_neurons,
  author    = {Anh Mai Nguyen and
               Alexey Dosovitskiy and
               Jason Yosinski and
               Thomas Brox and
               Jeff Clune},
  editor    = {Daniel D. Lee and
               Masashi Sugiyama and
               Ulrike von Luxburg and
               Isabelle Guyon and
               Roman Garnett},
  title     = {Synthesizing the preferred inputs for neurons in neural networks via
               deep generator networks},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {3387--3395},
  year      = {2016},
  url       = {http://papers.nips.cc/paper/6519-synthesizing-the-preferred-inputs-for-neurons-in-neural-networks-via-deep-generator-networks},
  timestamp = {Fri, 06 Mar 2020 17:00:38 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/NguyenDYBC16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{object_detectors_emerge_in_deep_scene_cnns,
  author    = {Bolei Zhou and
               Aditya Khosla and
               {\`{A}}gata Lapedriza and
               Aude Oliva and
               Antonio Torralba},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Object Detectors Emerge in Deep Scene CNNs},
  booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
               San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
  year      = {2015},
  url       = {http://arxiv.org/abs/1412.6856},
  timestamp = {Wed, 17 Jul 2019 10:40:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/ZhouKLOT14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{learning_aligned_cross_modal_representations,
  author    = {Llu{\'{\i}}s Castrej{\'{o}}n and
               Yusuf Aytar and
               Carl Vondrick and
               Hamed Pirsiavash and
               Antonio Torralba},
  title     = {Learning Aligned Cross-Modal Representations from Weakly Aligned Data},
  booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016},
  pages     = {2940--2949},
  publisher = {{IEEE} Computer Society},
  year      = {2016},
  url       = {https://doi.org/10.1109/CVPR.2016.321},
  doi       = {10.1109/CVPR.2016.321},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/CastrejonAVPT16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{measuring_association_between,
  title={Measuring Association Between Labels and Free-Text Rationales},
  author={Wiegreffe, Sarah and Marasovic, Ana and Smith, Noah A},
  journal={arXiv preprint arXiv:2010.12762},
  year={2020}
}

@article{opportunities_and_challenges_in_xai_survey,
  author    = {Arun Das and
               Paul Rad},
  title     = {Opportunities and Challenges in Explainable Artificial Intelligence
               {(XAI):} {A} Survey},
  journal   = {CoRR},
  volume    = {abs/2006.11371},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.11371},
  archivePrefix = {arXiv},
  eprint    = {2006.11371},
  timestamp = {Sat, 05 Sep 2020 17:48:52 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-11371.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{learning_3D_aware,
  author    = {Chengxi Li and
               Yue Meng and
               Stanley H. Chan and
               Yi{-}Ting Chen},
  title     = {Learning 3D-aware Egocentric Spatial-Temporal Interaction via Graph
               Convolutional Networks},
  booktitle = {2020 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2020, Paris, France, May 31 - August 31, 2020},
  pages     = {8418--8424},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/ICRA40945.2020.9197057},
  doi       = {10.1109/ICRA40945.2020.9197057},
  timestamp = {Mon, 28 Sep 2020 12:19:28 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/0006MCC20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{contrastive_explanation_structural,
  author    = {Tim Miller},
  title     = {Contrastive Explanation: {A} Structural-Model Approach},
  journal   = {CoRR},
  volume    = {abs/1811.03163},
  year      = {2018},
  url       = {http://arxiv.org/abs/1811.03163},
  archivePrefix = {arXiv},
  eprint    = {1811.03163},
  timestamp = {Thu, 22 Nov 2018 17:58:30 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1811-03163.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{counterfactual_explanation_without_opening,
  author    = {Sandra Wachter and
               Brent D. Mittelstadt and
               Chris Russell},
  title     = {Counterfactual Explanations without Opening the Black Box: Automated
               Decisions and the {GDPR}},
  journal   = {CoRR},
  volume    = {abs/1711.00399},
  year      = {2017},
  url       = {http://arxiv.org/abs/1711.00399},
  archivePrefix = {arXiv},
  eprint    = {1711.00399},
  timestamp = {Wed, 23 Jan 2019 13:31:00 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1711-00399.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{multi_objective_counterfactual_explanations,
  author    = {Susanne Dandl and
               Christoph Molnar and
               Martin Binder and
               Bernd Bischl},
  editor    = {Thomas B{\"{a}}ck and
               Mike Preuss and
               Andr{\'{e}} H. Deutz and
               Hao Wang and
               Carola Doerr and
               Michael T. M. Emmerich and
               Heike Trautmann},
  title     = {Multi-Objective Counterfactual Explanations},
  booktitle = {Parallel Problem Solving from Nature - {PPSN} {XVI} - 16th International
               Conference, {PPSN} 2020, Leiden, The Netherlands, September 5-9, 2020,
               Proceedings, Part {I}},
  series    = {Lecture Notes in Computer Science},
  volume    = {12269},
  pages     = {448--469},
  publisher = {Springer},
  year      = {2020},
  url       = {https://doi.org/10.1007/978-3-030-58112-1\_31},
  doi       = {10.1007/978-3-030-58112-1\_31},
  timestamp = {Wed, 21 Oct 2020 14:22:01 +0200},
  biburl    = {https://dblp.org/rec/conf/ppsn/DandlMBB20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{intriguing_properties_nn,
  author    = {Christian Szegedy and
               Wojciech Zaremba and
               Ilya Sutskever and
               Joan Bruna and
               Dumitru Erhan and
               Ian J. Goodfellow and
               Rob Fergus},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Intriguing properties of neural networks},
  booktitle = {2nd International Conference on Learning Representations, {ICLR} 2014,
               Banff, AB, Canada, April 14-16, 2014, Conference Track Proceedings},
  year      = {2014},
  url       = {http://arxiv.org/abs/1312.6199},
  timestamp = {Thu, 25 Jul 2019 14:35:25 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/SzegedyZSBEGF13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{ribeiro2018anchors,
  title={Anchors: High-Precision Model-Agnostic Explanations.},
  author={Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  year={2018}
}

@inproceedings{sato2001rule,
  title={Rule extraction from neural networks via decision tree induction},
  author={Sato, Makoto and Tsukimoto, Hiroshi},
  booktitle={IJCNN'01. International Joint Conference on Neural Networks. Proceedings (Cat. No. 01CH37222)},
  volume={3},
  pages={1870--1875},
  year={2001},
  organization={IEEE}
}

@inproceedings{DORN,
  author    = {Huan Fu and
               Mingming Gong and
               Chaohui Wang and
               Kayhan Batmanghelich and
               Dacheng Tao},
  title     = {Deep Ordinal Regression Network for Monocular Depth Estimation},
  booktitle = CVPR,
  npages     = {2002--2011},
  npublisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Fu\_Deep\_Ordinal\_Regression\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPR.2018.00214},
  timestamp = {Sat, 30 May 2020 20:05:36 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/FuGWBT18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Kuznietsov,
  author    = {Yevhen Kuznietsov and
               J{\"{o}}rg St{\"{u}}ckler and
               Bastian Leibe},
  title     = {Semi-Supervised Deep Learning for Monocular Depth Map Prediction},
  booktitle = CVPR,
  npages     = {2215--2223},
  npublisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.238},
  doi       = {10.1109/CVPR.2017.238},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/KuznietsovSL17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{semidepth,
  author    = {Ali Jahani Amiri and
               Shing Yan Loo and
               Hong Zhang},
  title     = {Semi-Supervised Monocular Depth Estimation with Left-Right Consistency
               Using Deep Neural Network},
  booktitle = {{IEEE} Int.\ Conf.\ Robotics and Biomimetics},
  npages     = {602--607},
  pnublisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ROBIO49542.2019.8961504},
  doi       = {10.1109/ROBIO49542.2019.8961504},
  timestamp = {Tue, 20 Oct 2020 14:11:38 +0200},
  biburl    = {https://dblp.org/rec/conf/robio/AmiriLZ19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{monodepth17,
  title     = {Unsupervised Monocular Depth Estimation with Left-Right Consistency},
  author    = {Cl{\'{e}}ment Godard and
               Oisin {Mac Aodha} and
               Gabriel J. Brostow},
  booktitle = CVPR,
  year = {2017}
}

@inproceedings{monodepth2,
  author    = {Cl{\'{e}}ment Godard and
               Oisin Mac Aodha and
               Michael Firman and
               Gabriel J. Brostow},
  title     = {Digging Into Self-Supervised Monocular Depth Estimation},
  booktitle = ICCV,
  npages     = {3827--3837},
  npublisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICCV.2019.00393},
  doi       = {10.1109/ICCV.2019.00393},
  timestamp = {Thu, 05 Mar 2020 13:43:22 +0100},
  biburl    = {https://dblp.org/rec/conf/iccv/GodardAFB19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{packnet,
  author = {Vitor Guizilini and Rares Ambrus and Sudeep Pillai and Allan Raventos and Adrien Gaidon},
  title = {{3D} Packing for Self-Supervised Monocular Depth Estimation},
  booktitle = CVPR,
  year = 2020
}

@inproceedings{Depth_Normal_Constraints,
  author    = {Yan Xu and
               Xinge Zhu and
               Jianping Shi and
               Guofeng Zhang and
               Hujun Bao and
               Hongsheng Li},
  title     = {Depth Completion From Sparse {LiDAR} Data With Depth-Normal Constraints},
  booktitle = ICCV,
  npages     = {2811--2820},
  npublisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICCV.2019.00290},
  doi       = {10.1109/ICCV.2019.00290},
  timestamp = {Thu, 05 Mar 2020 13:43:22 +0100},
  biburl    = {https://dblp.org/rec/conf/iccv/XuZS0BL19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{guided_depth_completion,
  author    = {Jie Tang and
               Fei{-}Peng Tian and
               Wei Feng and
               Jian Li and
               Ping Tan},
  title     = {Learning Guided Convolutional Network for Depth Completion},
  journal   = {CoRR},
  volume    = {abs/1908.01238},
  year      = {2019},
  url       = {http://arxiv.org/abs/1908.01238},
  archivePrefix = {arXiv},
  eprint    = {1908.01238},
  timestamp = {Fri, 09 Aug 2019 12:15:56 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1908-01238.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{jaritz_sparse_and_dense,
  author    = {Maximilian Jaritz and
               Raoul de Charette and
               {\'{E}}milie Wirbel and
               Xavier Perrotton and
               Fawzi Nashashibi},
  title     = {Sparse and Dense Data with {CNNs}: {D}epth Completion and Semantic Segmentation},
  booktitle = {Int. Conf. 3D Vision},
  npages     = {52--60},
  npublisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {https://doi.org/10.1109/3DV.2018.00017},
  doi       = {10.1109/3DV.2018.00017},
  timestamp = {Wed, 16 Oct 2019 14:14:49 +0200},
  biburl    = {https://dblp.org/rec/conf/3dim/JaritzCWPN18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{non_local_spatial_propagation,
    title={Non-Local Spatial Propagation Network for Depth Completion},
    author={Park, Jinsun and Joo, Kyungdon and Hu, Zhe and Liu, Chi-Kuei and Kweon, In So},
    booktitle=ECCV,
    year={2020}
}

@inproceedings{sfm_learner,
    Author = {Zhou, Tinghui and Brown, Matthew and Snavely, Noah and Lowe, David G.},
    Title = {Unsupervised Learning of Depth and Ego-Motion from Video},
    Booktitle = CVPR,
    Year = {2017}
}

@inproceedings{struct2depth,
  title={Depth Prediction without the Sensors: Leveraging Structure for Unsupervised Learning from Monocular Videos},
  author={Casser, Vincent and Pirk, Soeren and Mahjourian, Reza and Angelova, Anelia},
  booktitle=AAAI,
  year={2019}
}

@inproceedings{struct2depth_motion,
title={Unsupervised Monocular Depth and Ego-Motion Learning with Structure and Semantics},
author={Casser, Vincent and Pirk, Soeren and Mahjourian, Reza and Angelova, Anelia},
booktitle=CVPRW,
year={2019}
}


@inproceedings{psmnet,
  title={Pyramid Stereo Matching Network},
  author={Chang, Jia-Ren and Chen, Yong-Sheng},
  booktitle=CVPR,
  npages={5410--5418},
  year={2018}
}

@inproceedings{kendall_stereo,
  author    = {Alex Kendall and
               Hayk Martirosyan and
               Saumitro Dasgupta and
               Peter Henry},
  title     = {End-to-End Learning of Geometry and Context for Deep Stereo Regression},
  booktitle = ICCV,
  npages     = {66--75},
  npublisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/ICCV.2017.17},
  doi       = {10.1109/ICCV.2017.17},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iccv/KendallMDH17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{faster_rcnn,
  title={Faster r-cnn: Towards real-time object detection with region proposal networks},
  author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  booktitle={Advances in neural information processing systems},
  pages={91--99},
  year={2015}
}

@inproceedings{yolo,
  author    = {Joseph Redmon and
               Santosh Kumar Divvala and
               Ross B. Girshick and
               Ali Farhadi},
  title     = {You Only Look Once: Unified, Real-Time Object Detection},
  booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016},
  pages     = {779--788},
  publisher = {{IEEE} Computer Society},
  year      = {2016},
  url       = {https://doi.org/10.1109/CVPR.2016.91},
  doi       = {10.1109/CVPR.2016.91},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/RedmonDGF16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{yolov2_vehicle_detection,
  title={An improved YOLOv2 for vehicle detection},
  author={Sang, Jun and Wu, Zhongyuan and Guo, Pei and Hu, Haibo and Xiang, Hong and Zhang, Qian and Cai, Bin},
  journal={Sensors},
  volume={18},
  number={12},
  pages={4272},
  year={2018},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{yolov2,
  author    = {Joseph Redmon and
               Ali Farhadi},
  title     = {{YOLO9000:} Better, Faster, Stronger},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {6517--6525},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.690},
  doi       = {10.1109/CVPR.2017.690},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/RedmonF17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{yolov3,
  author    = {Joseph Redmon and
               Ali Farhadi},
  title     = {YOLOv3: An Incremental Improvement},
  journal   = {CoRR},
  volume    = {abs/1804.02767},
  year      = {2018},
  url       = {http://arxiv.org/abs/1804.02767},
  archivePrefix = {arXiv},
  eprint    = {1804.02767},
  timestamp = {Mon, 13 Aug 2018 16:48:24 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1804-02767.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{survey_object_detection_semantic_segmentation,
  author    = {Di Feng and
               Christian Haase{-}Sch{\"{u}}tz and
               Lars Rosenbaum and
               Heinz Hertlein and
               Fabian Duffhauss and
               Claudius Gl{\"{a}}ser and
               Werner Wiesbeck and
               Klaus Dietmayer},
  title     = {Deep Multi-modal Object Detection and Semantic Segmentation for Autonomous
               Driving: Datasets, Methods, and Challenges},
  journal   = {CoRR},
  volume    = {abs/1902.07830},
  year      = {2019},
  url       = {http://arxiv.org/abs/1902.07830},
  archivePrefix = {arXiv},
  eprint    = {1902.07830},
  timestamp = {Tue, 24 Nov 2020 17:45:29 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1902-07830.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{deep_learning_traffic_lights,
  author    = {Karsten Behrendt and
               Libor Novak and
               Rami Botros},
  title     = {A deep learning approach to traffic lights: Detection, tracking, and
               classification},
  booktitle = {2017 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2017, Singapore, Singapore, May 29 - June 3, 2017},
  pages     = {1370--1377},
  publisher = {{IEEE}},
  year      = {2017},
  url       = {https://doi.org/10.1109/ICRA.2017.7989163},
  doi       = {10.1109/ICRA.2017.7989163},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/BehrendtNB17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{stereo_vision_tracking,
  author    = {Peiliang Li and
               Tong Qin and
               Shaojie Shen},
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {Stereo Vision-Based Semantic 3D Object and Ego-Motion Tracking for
               Autonomous Driving},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {II}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11206},
  pages     = {664--679},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-01216-8\_40},
  doi       = {10.1007/978-3-030-01216-8\_40},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/LiQS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{PatroAN20,
  author    = {Badri N. Patro and
               Anupriy and
               Vinay Namboodiri},
  title     = {Explanation vs Attention: {A} Two-Player Game to Obtain Attention
               for {VQA}},
  booktitle = {The Thirty-Fourth {AAAI} Conference on Artificial Intelligence, {AAAI}
               2020, The Thirty-Second Innovative Applications of Artificial Intelligence
               Conference, {IAAI} 2020, The Tenth {AAAI} Symposium on Educational
               Advances in Artificial Intelligence, {EAAI} 2020, New York, NY, USA,
               February 7-12, 2020},
  pages     = {11848--11855},
  publisher = {{AAAI} Press},
  year      = {2020},
  url       = {https://aaai.org/ojs/index.php/AAAI/article/view/6858},
  timestamp = {Wed, 03 Jun 2020 18:42:45 +0200},
  biburl    = {https://dblp.org/rec/conf/aaai/PatroAN20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{predicting_pedestrian_intention,
  author    = {Karam M. Abughalieh and
               Shadi G. Alawneh},
  title     = {Predicting Pedestrian Intention to Cross the Road},
  journal   = {{IEEE} Access},
  volume    = {8},
  pages     = {72558--72569},
  year      = {2020},
  url       = {https://doi.org/10.1109/ACCESS.2020.2987777},
  doi       = {10.1109/ACCESS.2020.2987777},
  timestamp = {Mon, 15 Jun 2020 16:52:11 +0200},
  biburl    = {https://dblp.org/rec/journals/access/AbughaliehA20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pie_pedetrian_intention,
  author    = {Amir Rasouli and
               Iuliia Kotseruba and
               Toni Kunic and
               John K. Tsotsos},
  title     = {{PIE:} {A} Large-Scale Dataset and Models for Pedestrian Intention
               Estimation and Trajectory Prediction},
  booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
               2019, Seoul, Korea (South), October 27 - November 2, 2019},
  pages     = {6261--6270},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICCV.2019.00636},
  doi       = {10.1109/ICCV.2019.00636},
  timestamp = {Thu, 05 Mar 2020 13:43:22 +0100},
  biburl    = {https://dblp.org/rec/conf/iccv/RasouliKKT19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{differences_human_machine_perception,
  author    = {Taro Makino and
               Stanislaw Jastrzebski and
               Witold Oleszkiewicz and
               Celin Chacko and
               Robin Ehrenpreis and
               Naziya Samreen and
               Chloe Chhor and
               Eric Kim and
               Jiyon Lee and
               Kristine Pysarenko and
               Beatriu Reig and
               Hildegard Toth and
               Divya Awal and
               Linda Du and
               Alice Kim and
               James Park and
               Daniel K. Sodickson and
               Laura Heacock and
               Linda Moy and
               Kyunghyun Cho and
               Krzysztof J. Geras},
  title     = {Differences between human and machine perception in medical diagnosis},
  journal   = {CoRR},
  volume    = {abs/2011.14036},
  year      = {2020},
  url       = {https://arxiv.org/abs/2011.14036},
  archivePrefix = {arXiv},
  eprint    = {2011.14036},
  timestamp = {Tue, 01 Dec 2020 14:59:59 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2011-14036.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{cider,
  author    = {Ramakrishna Vedantam and
               C. Lawrence Zitnick and
               Devi Parikh},
  title     = {CIDEr: Consensus-based image description evaluation},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2015, Boston, MA, USA, June 7-12, 2015},
  pages     = {4566--4575},
  year      = {2015},
  crossref  = {DBLP:conf/cvpr/2015},
  url       = {https://doi.org/10.1109/CVPR.2015.7299087},
  doi       = {10.1109/CVPR.2015.7299087},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/VedantamZP15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{towards_faithfully_interpretable_nlp,
  author    = {Alon Jacovi and
               Yoav Goldberg},
  editor    = {Dan Jurafsky and
               Joyce Chai and
               Natalie Schluter and
               Joel R. Tetreault},
  title     = {Towards Faithfully Interpretable {NLP} Systems: How Should We Define
               and Evaluate Faithfulness?},
  booktitle = {Proceedings of the 58th Annual Meeting of the Association for Computational
               Linguistics, {ACL} 2020, Online, July 5-10, 2020},
  pages     = {4198--4205},
  publisher = {Association for Computational Linguistics},
  year      = {2020},
  url       = {https://www.aclweb.org/anthology/2020.acl-main.386/},
  timestamp = {Wed, 24 Jun 2020 17:15:07 +0200},
  biburl    = {https://dblp.org/rec/conf/acl/JacoviG20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{murel,
  author    = {R{\'{e}}mi Cad{\`{e}}ne and
               Hedi Ben{-}younes and
               Matthieu Cord and
               Nicolas Thome},
  title     = {{MUREL:} Multimodal Relational Reasoning for Visual Question Answering},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {1989--1998},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Cadene\_MUREL\_Multimodal\_Relational\_Reasoning\_for\_Visual\_Question\_Answering\_CVPR\_2019\_paper.html},
  doi       = {10.1109/CVPR.2019.00209},
  timestamp = {Thu, 27 Aug 2020 07:31:34 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/CadeneBCT19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{rubi,
  author    = {R{\'{e}}mi Cad{\`{e}}ne and
               Corentin Dancette and
               Hedi Ben{-}younes and
               Matthieu Cord and
               Devi Parikh},
  editor    = {Hanna M. Wallach and
               Hugo Larochelle and
               Alina Beygelzimer and
               Florence d'Alch{\'{e}}{-}Buc and
               Emily B. Fox and
               Roman Garnett},
  title     = {RUBi: Reducing Unimodal Biases for Visual Question Answering},
  booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
               on Neural Information Processing Systems 2019, NeurIPS 2019, December
               8-14, 2019, Vancouver, BC, Canada},
  pages     = {839--850},
  year      = {2019},
  url       = {http://papers.nips.cc/paper/8371-rubi-reducing-unimodal-biases-for-visual-question-answering},
  timestamp = {Tue, 01 Dec 2020 14:58:58 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/CadeneDBCP19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{clevr,
  author    = {Justin Johnson and
               Bharath Hariharan and
               Laurens van der Maaten and
               Li Fei{-}Fei and
               C. Lawrence Zitnick and
               Ross B. Girshick},
  title     = {{CLEVR:} {A} Diagnostic Dataset for Compositional Language and Elementary
               Visual Reasoning},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {1988--1997},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.215},
  doi       = {10.1109/CVPR.2017.215},
  timestamp = {Sat, 30 May 2020 20:05:36 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/JohnsonHMFZG17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{learning_to_reason,
  author    = {Ronghang Hu and
               Jacob Andreas and
               Marcus Rohrbach and
               Trevor Darrell and
               Kate Saenko},
  title     = {Learning to Reason: End-to-End Module Networks for Visual Question
               Answering},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2017, Venice,
               Italy, October 22-29, 2017},
  pages     = {804--813},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/ICCV.2017.93},
  doi       = {10.1109/ICCV.2017.93},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iccv/HuARDS17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{vqa_e,
  author    = {Qing Li and
               Qingyi Tao and
               Shafiq R. Joty and
               Jianfei Cai and
               Jiebo Luo},
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {{VQA-E:} Explaining, Elaborating, and Enhancing Your Answers for Visual
               Questions},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {VII}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11211},
  pages     = {570--586},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-01234-2\_34},
  doi       = {10.1007/978-3-030-01234-2\_34},
  timestamp = {Wed, 10 Jun 2020 15:40:49 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/LiTJCL18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{explaining_vqa_predictions,
  author    = {Felipe Riquelme and
               Alfredo De Goyeneche and
               Yundong Zhang and
               Juan Carlos Niebles and
               Alvaro Soto},
  title     = {Explaining {VQA} predictions using visual grounding and a knowledge
               base},
  journal   = {Image Vis. Comput.},
  volume    = {101},
  pages     = {103968},
  year      = {2020},
  url       = {https://doi.org/10.1016/j.imavis.2020.103968},
  doi       = {10.1016/j.imavis.2020.103968},
  timestamp = {Thu, 01 Oct 2020 09:25:48 +0200},
  biburl    = {https://dblp.org/rec/journals/ivc/RiquelmeGZNS20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{dont_just_assume,
  author    = {Aishwarya Agrawal and
               Dhruv Batra and
               Devi Parikh and
               Aniruddha Kembhavi},
  title     = {Don't Just Assume; Look and Answer: Overcoming Priors for Visual Question
               Answering},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {4971--4980},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Agrawal\_Dont\_Just\_Assume\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPR.2018.00522},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/AgrawalBPK18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{overcoming_language_priors,
  author    = {Sainandan Ramakrishnan and
               Aishwarya Agrawal and
               Stefan Lee},
  editor    = {Samy Bengio and
               Hanna M. Wallach and
               Hugo Larochelle and
               Kristen Grauman and
               Nicol{\`{o}} Cesa{-}Bianchi and
               Roman Garnett},
  title     = {Overcoming Language Priors in Visual Question Answering with Adversarial
               Regularization},
  booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
               on Neural Information Processing Systems 2018, NeurIPS 2018, December
               3-8, 2018, Montr{\'{e}}al, Canada},
  pages     = {1548--1558},
  year      = {2018},
  url       = {http://papers.nips.cc/paper/7427-overcoming-language-priors-in-visual-question-answering-with-adversarial-regularization},
  timestamp = {Tue, 01 Dec 2020 14:58:58 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/RamakrishnanAL18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{unbiased_look_dataset_bias,
  title={Unbiased look at dataset bias},
  author={Torralba, Antonio and Efros, Alexei A},
  booktitle={CVPR 2011},
  pages={1521--1528},
  year={2011},
  organization={IEEE}
}

@INPROCEEDINGS{bridging_day_night,
  author={E. {Romera} and L. M. {Bergasa} and K. {Yang} and J. M. {Alvarez} and R. {Barea}},
  booktitle={2019 IEEE Intelligent Vehicles Symposium (IV)}, 
  title={Bridging the Day and Night Domain Gap for Semantic Segmentation}, 
  year={2019},
  volume={},
  number={},
  pages={1312-1318},
  doi={10.1109/IVS.2019.8813888}
  }

@inproceedings{flow_edge_guided,
  author    = {Chen Gao and
               Ayush Saraf and
               Jia{-}Bin Huang and
               Johannes Kopf},
  editor    = {Andrea Vedaldi and
               Horst Bischof and
               Thomas Brox and
               Jan{-}Michael Frahm},
  title     = {Flow-edge Guided Video Completion},
  booktitle = {Computer Vision - {ECCV} 2020 - 16th European Conference, Glasgow,
               UK, August 23-28, 2020, Proceedings, Part {XII}},
  series    = {Lecture Notes in Computer Science},
  volume    = {12357},
  pages     = {713--729},
  publisher = {Springer},
  year      = {2020},
  url       = {https://doi.org/10.1007/978-3-030-58610-2\_42},
  doi       = {10.1007/978-3-030-58610-2\_42},
  timestamp = {Wed, 07 Oct 2020 19:50:13 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/GaoSHK20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
} 

@inproceedings{mocogan,
  author    = {Sergey Tulyakov and
               Ming{-}Yu Liu and
               Xiaodong Yang and
               Jan Kautz},
  title     = {MoCoGAN: Decomposing Motion and Content for Video Generation},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {1526--1535},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Tulyakov\_MoCoGAN\_Decomposing\_Motion\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPR.2018.00165},
  timestamp = {Fri, 20 Nov 2020 15:44:17 +0100},
  biburl    = {https://dblp.org/rec/conf/cvpr/Tulyakov0YK18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{recycle_gan,
  author    = {Aayush Bansal and
               Shugao Ma and
               Deva Ramanan and
               Yaser Sheikh},
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {Recycle-GAN: Unsupervised Video Retargeting},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {V}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11209},
  pages     = {122--138},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-01228-1\_8},
  doi       = {10.1007/978-3-030-01228-1\_8},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/BansalMRS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{optical_flow_distillation,
  author    = {Xinghao Chen and
               Yiman Zhang and
               Yunhe Wang and
               Han Shu and
               Chunjing Xu and
               Chang Xu},
  editor    = {Andrea Vedaldi and
               Horst Bischof and
               Thomas Brox and
               Jan{-}Michael Frahm},
  title     = {Optical Flow Distillation: Towards Efficient and Stable Video Style
               Transfer},
  booktitle = {Computer Vision - {ECCV} 2020 - 16th European Conference, Glasgow,
               UK, August 23-28, 2020, Proceedings, Part {VI}},
  series    = {Lecture Notes in Computer Science},
  volume    = {12351},
  pages     = {614--630},
  publisher = {Springer},
  year      = {2020},
  url       = {https://doi.org/10.1007/978-3-030-58539-6\_37},
  doi       = {10.1007/978-3-030-58539-6\_37},
  timestamp = {Tue, 17 Nov 2020 12:22:35 +0100},
  biburl    = {https://dblp.org/rec/conf/eccv/0001ZWSX020.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{vornet,
  author    = {Ya{-}Liang Chang and
               Zhe Yu Liu and
               Winston H. Hsu},
  title     = {VORNet: Spatio-Temporally Consistent Video Inpainting for Object Removal},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition Workshops,
               {CVPR} Workshops 2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {1785--1794},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPRW\_2019/html/NTIRE/Chang\_VORNet\_Spatio-Temporally\_Consistent\_Video\_Inpainting\_for\_Object\_Removal\_CVPRW\_2019\_paper.html},
  doi       = {10.1109/CVPRW.2019.00229},
  timestamp = {Mon, 20 Apr 2020 17:11:42 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/ChangLH19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{gan_augmentation,
  author    = {Christopher Bowles and
               Liang Chen and
               Ricardo Guerrero and
               Paul Bentley and
               Roger N. Gunn and
               Alexander Hammers and
               David Alexander Dickie and
               Maria del C. Vald{\'{e}}s Hern{\'{a}}ndez and
               Joanna M. Wardlaw and
               Daniel Rueckert},
  title     = {{GAN} Augmentation: Augmenting Training Data using Generative Adversarial
               Networks},
  journal   = {CoRR},
  volume    = {abs/1810.10863},
  year      = {2018},
  url       = {http://arxiv.org/abs/1810.10863},
  archivePrefix = {arXiv},
  eprint    = {1810.10863},
  timestamp = {Mon, 20 May 2019 16:58:37 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1810-10863.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{red_blood_cell,
  author    = {Oleksandr Bailo and
               DongShik Ham and
               Young Min Shin},
  title     = {Red Blood Cell Image Generation for Data Augmentation Using Conditional
               Generative Adversarial Networks},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition Workshops,
               {CVPR} Workshops 2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {1039--1048},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPRW\_2019/html/CVMI/Bailo\_Red\_Blood\_Cell\_Image\_Generation\_for\_Data\_Augmentation\_Using\_Conditional\_CVPRW\_2019\_paper.html},
  doi       = {10.1109/CVPRW.2019.00136},
  timestamp = {Mon, 20 Apr 2020 17:11:42 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/BailoHS19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{fadernet,
  author    = {Guillaume Lample and
               Neil Zeghidour and
               Nicolas Usunier and
               Antoine Bordes and
               Ludovic Denoyer and
               Marc'Aurelio Ranzato},
  editor    = {Isabelle Guyon and
               Ulrike von Luxburg and
               Samy Bengio and
               Hanna M. Wallach and
               Rob Fergus and
               S. V. N. Vishwanathan and
               Roman Garnett},
  title     = {Fader Networks: Manipulating Images by Sliding Attributes},
  booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
               on Neural Information Processing Systems 2017, December 4-9, 2017,
               Long Beach, CA, {USA}},
  pages     = {5967--5976},
  year      = {2017},
  url       = {http://papers.nips.cc/paper/7178-fader-networksmanipulating-images-by-sliding-attributes},
  timestamp = {Tue, 01 Dec 2020 14:58:58 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/LampleZUBDR17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{li2020causal,
    title={Causal discovery in physical systems from videos},
    author={Li, Yunzhu and Torralba, Antonio and Anandkumar, Anima and Fox, Dieter and Garg, Animesh},
    journal={Advances in Neural Information Processing Systems},
    volume={33},
    year={2020}
}
@misc{beef,
      title={Driving Behavior Explanation with Multi-level Fusion}, 
      author={Hédi Ben-Younes and Éloi Zablocki and Patrick Pérez and Matthieu Cord},
      year={2020},
      eprint={2012.04983},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}
@inproceedings{ben2019block,
  title={Block: Bilinear superdiagonal fusion for visual question answering and visual relationship detection},
  author={Ben-Younes, Hedi and Cadene, Remi and Thome, Nicolas and Cord, Matthieu},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  pages={8102--8109},
  year={2019}
}


